Computations of classical Mahowald invariants at prime 2

We review the definition of Mahowald invariants and discuss the computational method of Mark Brehens introduced in [arXiv:math/0507182]. Then we examine the relationship between the algebraic Mahowald invariants and the \( E \)-filtered Mahowald invariants, and compute the Mahowald invariants for most elements up to the 26-stem.

==> deleted.tex <==
\subsection{$M(4)$}
Let $C_2$ denote the cofiber of $2:S^0\rightarrow S^0$.
\begin{lemma}
$\pi_2C_2=\Z_4$ and $2\cdot\eta[1]=\eta^2[0]$ in $\pi_2C_2$.
\end{lemma}
\begin{proof}
By the long exact sequence of homotopy groups:
\[
\begin{tikzcd}
\pi_2S^0 \arrow[r, "2"] \arrow[d, no head, Rightarrow] & \pi_2S^0 \arrow[r] \arrow[d, no head, Rightarrow] & \pi_2C_2 \arrow[r] & \pi_2S^1 \arrow[r, "2"] \arrow[d, no head, Rightarrow] & \pi_2S^1 \arrow[d, no head, Rightarrow] \\
\Z_2\{\eta^2\} \arrow[r, "2"]                  & \Z_2\{\eta^2\}                            &                    & \Z_2\{\eta\} \arrow[r, "2"]                         & \Z_2\{\eta\}                   
\end{tikzcd}
\]
we know $\pi_2C_2$ is $\Z_4$ or $\Z_2\times\Z_2$.

We only need to show a nontrivial extension: $2\cdot\eta[1]=\eta^2[0]$ in $\pi_2C_2$. Since
\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Ellipse [id:dp4596375963182404] 
\draw   (55,172.39) .. controls (55,169.72) and (57.2,167.56) .. (59.91,167.56) .. controls (62.62,167.56) and (64.82,169.72) .. (64.82,172.39) .. controls (64.82,175.06) and (62.62,177.23) .. (59.91,177.23) .. controls (57.2,177.23) and (55,175.06) .. (55,172.39) -- cycle ;
%Shape: Ellipse [id:dp009483521811293638] 
\draw   (367.93,179.03) .. controls (366.54,181.31) and (363.52,182.05) .. (361.2,180.67) .. controls (358.87,179.3) and (358.12,176.33) .. (359.52,174.04) .. controls (360.92,171.76) and (363.94,171.02) .. (366.26,172.4) .. controls (368.58,173.77) and (369.33,176.74) .. (367.93,179.03) -- cycle ;
%Shape: Ellipse [id:dp567200132046155] 
\draw   (367.93,210.51) .. controls (366.54,212.79) and (363.52,213.53) .. (361.2,212.16) .. controls (358.87,210.78) and (358.12,207.81) .. (359.52,205.52) .. controls (360.92,203.24) and (363.94,202.5) .. (366.26,203.88) .. controls (368.58,205.25) and (369.33,208.22) .. (367.93,210.51) -- cycle ;
%Shape: Ellipse [id:dp6660379899683821] 
\draw   (321.65,210.51) .. controls (320.25,212.79) and (317.23,213.53) .. (314.91,212.16) .. controls (312.58,210.78) and (311.84,207.81) .. (313.23,205.52) .. controls (314.63,203.24) and (317.65,202.5) .. (319.97,203.88) .. controls (322.3,205.25) and (323.04,208.22) .. (321.65,210.51) -- cycle ;
%Shape: Ellipse [id:dp07981907848339453] 
\draw   (273.67,210.51) .. controls (272.28,212.79) and (269.26,213.53) .. (266.94,212.16) .. controls (264.61,210.78) and (263.86,207.81) .. (265.26,205.52) .. controls (266.66,203.24) and (269.68,202.5) .. (272,203.88) .. controls (274.32,205.25) and (275.07,208.22) .. (273.67,210.51) -- cycle ;
%Shape: Ellipse [id:dp37935306381689804] 
\draw   (273.67,178.2) .. controls (272.28,180.49) and (269.26,181.22) .. (266.94,179.85) .. controls (264.61,178.47) and (263.86,175.5) .. (265.26,173.21) .. controls (266.66,170.93) and (269.68,170.19) .. (272,171.57) .. controls (274.32,172.94) and (275.07,175.91) .. (273.67,178.2) -- cycle ;
%Shape: Ellipse [id:dp47156272361789875] 
\draw   (223.18,179.03) .. controls (221.78,181.31) and (218.76,182.05) .. (216.44,180.67) .. controls (214.12,179.3) and (213.37,176.33) .. (214.77,174.04) .. controls (216.17,171.76) and (219.18,171.02) .. (221.51,172.4) .. controls (223.83,173.77) and (224.58,176.74) .. (223.18,179.03) -- cycle ;
%Shape: Ellipse [id:dp7534131854181136] 
\draw   (161.74,208.85) .. controls (160.34,211.14) and (157.33,211.88) .. (155,210.5) .. controls (152.68,209.12) and (151.93,206.15) .. (153.33,203.87) .. controls (154.73,201.58) and (157.75,200.84) .. (160.07,202.22) .. controls (162.39,203.6) and (163.14,206.57) .. (161.74,208.85) -- cycle ;
%Shape: Ellipse [id:dp9937918361796334] 
\draw   (161.74,175.71) .. controls (160.34,178) and (157.33,178.74) .. (155,177.36) .. controls (152.68,175.98) and (151.93,173.01) .. (153.33,170.73) .. controls (154.73,168.44) and (157.75,167.7) .. (160.07,169.08) .. controls (162.39,170.46) and (163.14,173.43) .. (161.74,175.71) -- cycle ;
%Shape: Ellipse [id:dp9647231699634229] 
\draw   (113.77,174.89) .. controls (112.37,177.17) and (109.35,177.91) .. (107.03,176.53) .. controls (104.71,175.16) and (103.96,172.19) .. (105.36,169.9) .. controls (106.76,167.61) and (109.77,166.88) .. (112.1,168.25) .. controls (114.42,169.63) and (115.17,172.6) .. (113.77,174.89) -- cycle ;
%Shape: Ellipse [id:dp5119150368707517] 
\draw   (511.15,176.54) .. controls (511.15,173.87) and (513.35,171.7) .. (516.06,171.7) .. controls (518.77,171.7) and (520.97,173.87) .. (520.97,176.54) .. controls (520.97,179.2) and (518.77,181.37) .. (516.06,181.37) .. controls (513.35,181.37) and (511.15,179.2) .. (511.15,176.54) -- cycle ;
%Shape: Ellipse [id:dp8970455585426202] 
\draw   (511.15,209.67) .. controls (511.15,207) and (513.35,204.84) .. (516.06,204.84) .. controls (518.77,204.84) and (520.97,207) .. (520.97,209.67) .. controls (520.97,212.34) and (518.77,214.5) .. (516.06,214.5) .. controls (513.35,214.5) and (511.15,212.34) .. (511.15,209.67) -- cycle ;
%Shape: Ellipse [id:dp4995656398357333] 
\draw   (464.86,208.84) .. controls (464.86,206.18) and (467.06,204.01) .. (469.77,204.01) .. controls (472.48,204.01) and (474.68,206.18) .. (474.68,208.84) .. controls (474.68,211.51) and (472.48,213.68) .. (469.77,213.68) .. controls (467.06,213.68) and (464.86,211.51) .. (464.86,208.84) -- cycle ;
%Shape: Ellipse [id:dp5258742335784536] 
\draw   (416.89,176.54) .. controls (416.89,173.87) and (419.09,171.7) .. (421.8,171.7) .. controls (424.51,171.7) and (426.71,173.87) .. (426.71,176.54) .. controls (426.71,179.2) and (424.51,181.37) .. (421.8,181.37) .. controls (419.09,181.37) and (416.89,179.2) .. (416.89,176.54) -- cycle ;
%Straight Lines [id:da09542885708759075] 
\draw    (64.82,172.39) -- (99.29,172.52) ;
\draw [shift={(101.29,172.53)}, rotate = 180.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5873348458176972] 
\draw    (118.12,173.36) -- (149.79,174.14) ;
\draw [shift={(151.78,174.19)}, rotate = 181.41] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8183078758232318] 
\draw    (158.37,177.36) -- (157.7,202.22) ;
%Straight Lines [id:da7009441974775534] 
\draw    (224.86,177.37) -- (263.26,176.57) ;
\draw [shift={(265.26,176.53)}, rotate = 178.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7141287762217432] 
\draw    (269.61,180.82) -- (268.64,202.22) ;
%Straight Lines [id:da07973895880907045] 
\draw    (273.67,208.85) -- (308.85,208.19) ;
\draw [shift={(310.85,208.15)}, rotate = 178.92] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5256693306700839] 
\draw    (363.72,182.33) -- (363.74,202.22) ;
%Curve Lines [id:da35305525152469786] 
\draw    (331.05,204.84) .. controls (313.64,210.55) and (323.04,207.28) .. (357.91,207.97) ;
\draw [shift={(359.52,208.01)}, rotate = 181.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08804778852326178] 
\draw    (425.87,179.85) -- (464.07,206.86) ;
\draw [shift={(465.7,208.02)}, rotate = 215.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da2880479949918333] 
\draw    (482.67,206.5) .. controls (465.26,212.22) and (474.67,208.95) .. (509.54,209.64) ;
\draw [shift={(511.15,209.67)}, rotate = 181.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5398949038355862] 
\draw    (516.06,181.37) -- (516.06,204.84) ;

% Text Node
\draw (76.01,160.68) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (127.35,159.11) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \eta $};
% Text Node
\draw (239.28,166.65) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (267.75,182.79) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \eta $};
% Text Node
\draw (286.41,198.13) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (187.94,177.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (394.14,181.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (362.47,186.05) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (516.03,186.54) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (439.79,173.94) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \eta ^{2}$};
% Text Node
\draw (157,187.36) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};


\end{tikzpicture}
\]
where the first equality is from Corollary 7.4 in the appendix and the second equality is Toda bracket $\langle2,\eta,2\rangle=\eta^2$, we know $2\cdot\eta[1]=\eta^2[0]$ and complete the proof.
\end{proof}

When $N=2$, $4\iota[-1]=2\cdot\eta[-2]=0$ and there is no other extension, so $4\iota[-1]$ is trivial in $\pi_{-1}(P^{\infty}_{-2})$. When $N=3$, by the following cofiber sequence:
\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Ellipse [id:dp25928281207519577] 
\draw   (174,151.96) .. controls (174,145.02) and (180.37,139.39) .. (188.23,139.39) .. controls (196.09,139.39) and (202.46,145.02) .. (202.46,151.96) .. controls (202.46,158.9) and (196.09,164.52) .. (188.23,164.52) .. controls (180.37,164.52) and (174,158.9) .. (174,151.96) -- cycle ;
%Shape: Ellipse [id:dp921532650431585] 
\draw   (368.21,202.96) .. controls (368.21,196.02) and (374.58,190.39) .. (382.44,190.39) .. controls (390.3,190.39) and (396.67,196.02) .. (396.67,202.96) .. controls (396.67,209.9) and (390.3,215.53) .. (382.44,215.53) .. controls (374.58,215.53) and (368.21,209.9) .. (368.21,202.96) -- cycle ;
%Shape: Ellipse [id:dp5030777206045209] 
\draw   (368.21,154.18) .. controls (368.21,147.24) and (374.58,141.61) .. (382.44,141.61) .. controls (390.3,141.61) and (396.67,147.24) .. (396.67,154.18) .. controls (396.67,161.12) and (390.3,166.74) .. (382.44,166.74) .. controls (374.58,166.74) and (368.21,161.12) .. (368.21,154.18) -- cycle ;
%Shape: Ellipse [id:dp4731779374129461] 
\draw   (302.91,162.31) .. controls (302.91,155.37) and (309.29,149.74) .. (317.15,149.74) .. controls (325,149.74) and (331.38,155.37) .. (331.38,162.31) .. controls (331.38,169.25) and (325,174.87) .. (317.15,174.87) .. controls (309.29,174.87) and (302.91,169.25) .. (302.91,162.31) -- cycle ;
%Straight Lines [id:da7597727353959274] 
\draw    (217.53,151.47) -- (272.45,152.18) ;
\draw [shift={(274.45,152.2)}, rotate = 180.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0069484289959163] 
\draw    (382.44,166.74) -- (382.44,190.39) ;
%Straight Lines [id:da4425967270863944] 
\draw    (415.92,164.03) -- (478.38,164.03) ;
\draw [shift={(480.38,164.03)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp7465278255689538] 
\draw   (513.86,219.56) .. controls (513.86,214.72) and (519.86,210.8) .. (527.26,210.8) .. controls (534.66,210.8) and (540.66,214.72) .. (540.66,219.56) .. controls (540.66,224.39) and (534.66,228.32) .. (527.26,228.32) .. controls (519.86,228.32) and (513.86,224.39) .. (513.86,219.56) -- cycle ;
%Shape: Ellipse [id:dp14883236758879304] 
\draw   (513.86,185.56) .. controls (513.86,180.73) and (519.86,176.81) .. (527.26,176.81) .. controls (534.66,176.81) and (540.66,180.73) .. (540.66,185.56) .. controls (540.66,190.4) and (534.66,194.32) .. (527.26,194.32) .. controls (519.86,194.32) and (513.86,190.4) .. (513.86,185.56) -- cycle ;
%Straight Lines [id:da3540345149374342] 
\draw    (527.26,194.32) -- (527.26,210.8) ;
%Shape: Ellipse [id:dp1984240490599012] 
\draw   (513.86,152.08) .. controls (513.86,147.25) and (519.86,143.33) .. (527.26,143.33) .. controls (534.66,143.33) and (540.66,147.25) .. (540.66,152.08) .. controls (540.66,156.92) and (534.66,160.84) .. (527.26,160.84) .. controls (519.86,160.84) and (513.86,156.92) .. (513.86,152.08) -- cycle ;
%Shape: Ellipse [id:dp38794190123557937] 
\draw   (513.86,118.09) .. controls (513.86,113.25) and (519.86,109.33) .. (527.26,109.33) .. controls (534.66,109.33) and (540.66,113.25) .. (540.66,118.09) .. controls (540.66,122.93) and (534.66,126.85) .. (527.26,126.85) .. controls (519.86,126.85) and (513.86,122.93) .. (513.86,118.09) -- cycle ;
%Straight Lines [id:da060370489459460996] 
\draw    (527.26,126.85) -- (527.26,143.33) ;
%Curve Lines [id:da2673960080332949] 
\draw    (540.66,118.09) .. controls (560.36,117.75) and (557.21,185.22) .. (540.66,185.56) ;

% Text Node
\draw (181.99,149) node [anchor=north west][inner sep=0.75pt]   [align=left] {\mbox{-}1};
% Text Node
\draw (310.06,159.35) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {\mbox{-}1};
% Text Node
\draw (377.03,151.96) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {\mbox{-}2};
% Text Node
\draw (376.19,200) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {\mbox{-}3};
% Text Node
\draw (229.5,134.09) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle 2\lor \eta $};
% Text Node
\draw (383.22,174.13) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {2};
% Text Node
\draw (521.73,181.44) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {\mbox{-}2};
% Text Node
\draw (521.95,214.92) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {\mbox{-}3};
% Text Node
\draw (527.67,196.89) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {2};
% Text Node
\draw (522.16,113.97) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {0};
% Text Node
\draw (520.95,147.45) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {\mbox{-}1};
% Text Node
\draw (527.67,129.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (542.65,140.51) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};


\end{tikzpicture},
\]
\qquad\quad
\begin{tikzcd}
{2\iota[-1]} \arrow[rrr, maps to] &  &  & {4\iota[-1]\oplus2\cdot\eta[-2]}
\end{tikzcd}

we know $4\iota[-1]=2\cdot\eta[-2]$ from the long exact sequence of homotopy groups, and $2\cdot\eta[-2]=\eta^2[-3]$ in $P^{0}_{-3}$ by Lemma 4.3, so $N=3$ and $M(4)=\eta^2$ by the fact $\pi_2=\Z_2\{\eta^2\}$.

\subsection{$M(\eta^2)$}

Since in the case ``$\eta$", we know $N=3$, we deduce that $N\geq3$ in the case ``$\eta^2$". Furthermore, we know $N\geq5$ because $\pi_4$ and $\pi_5$ are both trivial.

We compute $\pi_1(P^{\infty}_{-5})$ by the AHSS to find that $\pi_1(P^{\infty}_{-5})=\Z_2\{\nu^2[-5]\}$ since we have:
\[
d_1(\iota[2])=2\iota[1]\qquad d_1(\mu[-2])=2\cdot\mu[-3]
\]
\[
d_2(\eta[1])=\eta^2[-1] \qquad d_2(\eta[0])=\eta^2[-2] \qquad d_2(\eta^2[0])=\eta^3[-2]=4\nu[-2],
\]
Thus we obtain $\pi_1(P^{\infty}_{-5})=\Z_2\{\nu^2[-5]\}$.

By Lemma 7. in the appendix and $\langle\eta,\nu,\eta\rangle=\nu^2$, we have:

\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Ellipse [id:dp7465278255689538] 
\draw   (193.93,259.52) .. controls (193.93,255.78) and (198.2,252.76) .. (203.47,252.76) .. controls (208.75,252.76) and (213.02,255.78) .. (213.02,259.52) .. controls (213.02,263.25) and (208.75,266.27) .. (203.47,266.27) .. controls (198.2,266.27) and (193.93,263.25) .. (193.93,259.52) -- cycle ;
%Shape: Ellipse [id:dp14883236758879304] 
\draw   (193.93,233.28) .. controls (193.93,229.54) and (198.2,226.52) .. (203.47,226.52) .. controls (208.75,226.52) and (213.02,229.54) .. (213.02,233.28) .. controls (213.02,237.01) and (208.75,240.04) .. (203.47,240.04) .. controls (198.2,240.04) and (193.93,237.01) .. (193.93,233.28) -- cycle ;
%Straight Lines [id:da3540345149374342] 
\draw    (203.47,240.04) -- (203.47,252.76) ;
%Shape: Ellipse [id:dp1984240490599012] 
\draw   (193.93,207.44) .. controls (193.93,203.7) and (198.2,200.68) .. (203.47,200.68) .. controls (208.75,200.68) and (213.02,203.7) .. (213.02,207.44) .. controls (213.02,211.17) and (208.75,214.19) .. (203.47,214.19) .. controls (198.2,214.19) and (193.93,211.17) .. (193.93,207.44) -- cycle ;
%Shape: Ellipse [id:dp38794190123557937] 
\draw   (193.93,181.2) .. controls (193.93,177.46) and (198.2,174.44) .. (203.47,174.44) .. controls (208.75,174.44) and (213.02,177.46) .. (213.02,181.2) .. controls (213.02,184.93) and (208.75,187.96) .. (203.47,187.96) .. controls (198.2,187.96) and (193.93,184.93) .. (193.93,181.2) -- cycle ;
%Straight Lines [id:da060370489459460996] 
\draw    (203.47,187.96) -- (203.47,200.68) ;
%Curve Lines [id:da2673960080332949] 
\draw    (213.02,181.2) .. controls (227.07,180.93) and (224.82,233.01) .. (213.02,233.28) ;
%Shape: Ellipse [id:dp17242569052162948] 
\draw   (194.64,287.3) .. controls (194.64,283.57) and (198.91,280.54) .. (204.19,280.54) .. controls (209.46,280.54) and (213.74,283.57) .. (213.74,287.3) .. controls (213.74,291.04) and (209.46,294.06) .. (204.19,294.06) .. controls (198.91,294.06) and (194.64,291.04) .. (194.64,287.3) -- cycle ;
%Shape: Ellipse [id:dp8113090465797512] 
\draw   (194.64,318.18) .. controls (194.64,314.44) and (198.91,311.42) .. (204.19,311.42) .. controls (209.46,311.42) and (213.74,314.44) .. (213.74,318.18) .. controls (213.74,321.91) and (209.46,324.93) .. (204.19,324.93) .. controls (198.91,324.93) and (194.64,321.91) .. (194.64,318.18) -- cycle ;
%Straight Lines [id:da4488545808148945] 
\draw    (204.19,294.06) -- (204.19,311.42) ;
%Shape: Ellipse [id:dp22519635947625627] 
\draw   (193.93,153) .. controls (193.93,149.27) and (198.2,146.24) .. (203.47,146.24) .. controls (208.75,146.24) and (213.02,149.27) .. (213.02,153) .. controls (213.02,156.73) and (208.75,159.76) .. (203.47,159.76) .. controls (198.2,159.76) and (193.93,156.73) .. (193.93,153) -- cycle ;
%Curve Lines [id:da8478716169945162] 
\draw    (213.02,259.52) .. controls (227.07,259.25) and (224.82,315.6) .. (213.02,315.86) ;
%Curve Lines [id:da5145543113097282] 
\draw    (193.93,153) .. controls (189.03,150.6) and (176.92,204.63) .. (193.93,207.44) ;
%Curve Lines [id:da35319652222966536] 
\draw    (213.02,259.52) .. controls (235.36,260.2) and (234.65,152.91) .. (213.02,153) ;
%Shape: Ellipse [id:dp26357279955435] 
\draw   (395.82,254.81) .. controls (395.82,251.08) and (400.09,248.06) .. (405.37,248.06) .. controls (410.64,248.06) and (414.92,251.08) .. (414.92,254.81) .. controls (414.92,258.55) and (410.64,261.57) .. (405.37,261.57) .. controls (400.09,261.57) and (395.82,258.55) .. (395.82,254.81) -- cycle ;
%Shape: Ellipse [id:dp5896286547965521] 
\draw   (395.82,228.58) .. controls (395.82,224.84) and (400.09,221.82) .. (405.37,221.82) .. controls (410.64,221.82) and (414.92,224.84) .. (414.92,228.58) .. controls (414.92,232.31) and (410.64,235.33) .. (405.37,235.33) .. controls (400.09,235.33) and (395.82,232.31) .. (395.82,228.58) -- cycle ;
%Straight Lines [id:da23841153481138866] 
\draw    (405.37,235.33) -- (405.37,248.06) ;
%Shape: Ellipse [id:dp09488161825551367] 
\draw   (395.82,202.73) .. controls (395.82,199) and (400.09,195.98) .. (405.37,195.98) .. controls (410.64,195.98) and (414.92,199) .. (414.92,202.73) .. controls (414.92,206.47) and (410.64,209.49) .. (405.37,209.49) .. controls (400.09,209.49) and (395.82,206.47) .. (395.82,202.73) -- cycle ;
%Shape: Ellipse [id:dp2565825455491708] 
\draw   (395.82,176.5) .. controls (395.82,172.76) and (400.09,169.74) .. (405.37,169.74) .. controls (410.64,169.74) and (414.92,172.76) .. (414.92,176.5) .. controls (414.92,180.23) and (410.64,183.25) .. (405.37,183.25) .. controls (400.09,183.25) and (395.82,180.23) .. (395.82,176.5) -- cycle ;
%Straight Lines [id:da34234393307766675] 
\draw    (405.37,183.25) -- (405.37,195.98) ;
%Curve Lines [id:da367997919461869] 
\draw    (414.92,176.5) .. controls (428.96,176.23) and (426.71,228.31) .. (414.92,228.58) ;
%Shape: Ellipse [id:dp3494064029893562] 
\draw   (396.53,282.6) .. controls (396.53,278.87) and (400.81,275.84) .. (406.08,275.84) .. controls (411.35,275.84) and (415.63,278.87) .. (415.63,282.6) .. controls (415.63,286.33) and (411.35,289.36) .. (406.08,289.36) .. controls (400.81,289.36) and (396.53,286.33) .. (396.53,282.6) -- cycle ;
%Shape: Ellipse [id:dp8546191293571337] 
\draw   (396.53,313.48) .. controls (396.53,309.74) and (400.81,306.72) .. (406.08,306.72) .. controls (411.35,306.72) and (415.63,309.74) .. (415.63,313.48) .. controls (415.63,317.21) and (411.35,320.23) .. (406.08,320.23) .. controls (400.81,320.23) and (396.53,317.21) .. (396.53,313.48) -- cycle ;
%Straight Lines [id:da07407350153671466] 
\draw    (406.08,289.36) -- (406.08,306.72) ;
%Shape: Ellipse [id:dp5487292130852242] 
\draw   (395.82,148.3) .. controls (395.82,144.57) and (400.09,141.54) .. (405.37,141.54) .. controls (410.64,141.54) and (414.92,144.57) .. (414.92,148.3) .. controls (414.92,152.03) and (410.64,155.06) .. (405.37,155.06) .. controls (400.09,155.06) and (395.82,152.03) .. (395.82,148.3) -- cycle ;
%Curve Lines [id:da562459953803802] 
\draw    (414.92,254.81) .. controls (428.96,254.55) and (426.71,310.9) .. (414.92,311.16) ;
%Curve Lines [id:da6716767141913642] 
\draw    (395.82,148.3) .. controls (390.92,145.9) and (378.81,199.93) .. (395.82,202.73) ;
%Curve Lines [id:da11171248210168838] 
\draw    (414.92,254.81) .. controls (437.25,255.5) and (436.54,148.21) .. (414.92,148.3) ;
%Shape: Ellipse [id:dp04604564668102862] 
\draw   (569.27,254.81) .. controls (569.27,251.08) and (573.55,248.06) .. (578.82,248.06) .. controls (584.1,248.06) and (588.37,251.08) .. (588.37,254.81) .. controls (588.37,258.55) and (584.1,261.57) .. (578.82,261.57) .. controls (573.55,261.57) and (569.27,258.55) .. (569.27,254.81) -- cycle ;
%Shape: Ellipse [id:dp8768779358966419] 
\draw   (569.27,228.58) .. controls (569.27,224.84) and (573.55,221.82) .. (578.82,221.82) .. controls (584.1,221.82) and (588.37,224.84) .. (588.37,228.58) .. controls (588.37,232.31) and (584.1,235.33) .. (578.82,235.33) .. controls (573.55,235.33) and (569.27,232.31) .. (569.27,228.58) -- cycle ;
%Straight Lines [id:da6997795166467606] 
\draw    (578.82,235.33) -- (578.82,248.06) ;
%Shape: Ellipse [id:dp9684146514753416] 
\draw   (569.27,202.73) .. controls (569.27,199) and (573.55,195.98) .. (578.82,195.98) .. controls (584.1,195.98) and (588.37,199) .. (588.37,202.73) .. controls (588.37,206.47) and (584.1,209.49) .. (578.82,209.49) .. controls (573.55,209.49) and (569.27,206.47) .. (569.27,202.73) -- cycle ;
%Shape: Ellipse [id:dp3268535246066593] 
\draw   (569.27,176.5) .. controls (569.27,172.76) and (573.55,169.74) .. (578.82,169.74) .. controls (584.1,169.74) and (588.37,172.76) .. (588.37,176.5) .. controls (588.37,180.23) and (584.1,183.25) .. (578.82,183.25) .. controls (573.55,183.25) and (569.27,180.23) .. (569.27,176.5) -- cycle ;
%Straight Lines [id:da6332160264074236] 
\draw    (578.82,183.25) -- (578.82,195.98) ;
%Curve Lines [id:da6923846308904467] 
\draw    (588.37,176.5) .. controls (602.41,176.23) and (600.17,228.31) .. (588.37,228.58) ;
%Shape: Ellipse [id:dp2414906241614383] 
\draw   (569.99,282.6) .. controls (569.99,278.87) and (574.26,275.84) .. (579.54,275.84) .. controls (584.81,275.84) and (589.08,278.87) .. (589.08,282.6) .. controls (589.08,286.33) and (584.81,289.36) .. (579.54,289.36) .. controls (574.26,289.36) and (569.99,286.33) .. (569.99,282.6) -- cycle ;
%Shape: Ellipse [id:dp3331972183048404] 
\draw   (569.99,313.48) .. controls (569.99,309.74) and (574.26,306.72) .. (579.54,306.72) .. controls (584.81,306.72) and (589.08,309.74) .. (589.08,313.48) .. controls (589.08,317.21) and (584.81,320.23) .. (579.54,320.23) .. controls (574.26,320.23) and (569.99,317.21) .. (569.99,313.48) -- cycle ;
%Straight Lines [id:da5419882396849149] 
\draw    (579.54,289.36) -- (579.54,306.72) ;
%Shape: Ellipse [id:dp9083208103912579] 
\draw   (569.27,148.3) .. controls (569.27,144.57) and (573.55,141.54) .. (578.82,141.54) .. controls (584.1,141.54) and (588.37,144.57) .. (588.37,148.3) .. controls (588.37,152.03) and (584.1,155.06) .. (578.82,155.06) .. controls (573.55,155.06) and (569.27,152.03) .. (569.27,148.3) -- cycle ;
%Curve Lines [id:da03528731092351012] 
\draw    (588.37,254.81) .. controls (602.41,254.55) and (600.17,310.9) .. (588.37,311.16) ;
%Curve Lines [id:da8221814874362685] 
\draw    (569.27,148.3) .. controls (564.38,145.9) and (552.27,199.93) .. (569.27,202.73) ;
%Curve Lines [id:da163464063156886] 
\draw    (588.37,254.81) .. controls (610.71,255.5) and (609.99,148.21) .. (588.37,148.3) ;
%Shape: Ellipse [id:dp11580026283836298] 
\draw   (79,152.7) .. controls (79,148.97) and (83.28,145.94) .. (88.55,145.94) .. controls (93.82,145.94) and (98.1,148.97) .. (98.1,152.7) .. controls (98.1,156.43) and (93.82,159.46) .. (88.55,159.46) .. controls (83.28,159.46) and (79,156.43) .. (79,152.7) -- cycle ;
%Shape: Ellipse [id:dp881794400592975] 
\draw   (124.5,206.29) .. controls (124.5,202.56) and (128.77,199.53) .. (134.05,199.53) .. controls (139.32,199.53) and (143.59,202.56) .. (143.59,206.29) .. controls (143.59,210.02) and (139.32,213.05) .. (134.05,213.05) .. controls (128.77,213.05) and (124.5,210.02) .. (124.5,206.29) -- cycle ;
%Straight Lines [id:da3404074587290069] 
\draw    (88.55,159.46) -- (123.28,204.7) ;
\draw [shift={(124.5,206.29)}, rotate = 232.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da16079221604578153] 
\draw    (156.31,202.66) .. controls (134.72,211.03) and (140.08,208.35) .. (192.33,207.46) ;
\draw [shift={(193.93,207.44)}, rotate = 179.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp2232714074380926] 
\draw   (268.57,158.34) .. controls (268.57,154.61) and (272.85,151.58) .. (278.12,151.58) .. controls (283.39,151.58) and (287.67,154.61) .. (287.67,158.34) .. controls (287.67,162.07) and (283.39,165.1) .. (278.12,165.1) .. controls (272.85,165.1) and (268.57,162.07) .. (268.57,158.34) -- cycle ;
%Shape: Ellipse [id:dp8921239747234513] 
\draw   (335.8,254.42) .. controls (335.8,250.69) and (340.07,247.66) .. (345.35,247.66) .. controls (350.62,247.66) and (354.9,250.69) .. (354.9,254.42) .. controls (354.9,258.15) and (350.62,261.18) .. (345.35,261.18) .. controls (340.07,261.18) and (335.8,258.15) .. (335.8,254.42) -- cycle ;
%Straight Lines [id:da49048180917854634] 
\draw    (278.12,165.1) -- (337.12,246.17) ;
\draw [shift={(338.29,247.79)}, rotate = 233.96] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da707758848157898] 
\draw    (367.68,247.79) .. controls (350.79,250.58) and (345.97,263.51) .. (394.34,255.08) ;
\draw [shift={(395.82,254.81)}, rotate = 169.83] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp7585837733905549] 
\draw   (458.14,161.16) .. controls (458.14,157.43) and (462.42,154.4) .. (467.69,154.4) .. controls (472.96,154.4) and (477.24,157.43) .. (477.24,161.16) .. controls (477.24,164.89) and (472.96,167.92) .. (467.69,167.92) .. controls (462.42,167.92) and (458.14,164.89) .. (458.14,161.16) -- cycle ;
%Shape: Ellipse [id:dp8795927681803761] 
\draw   (520.63,313.65) .. controls (520.63,309.92) and (524.9,306.89) .. (530.18,306.89) .. controls (535.45,306.89) and (539.73,309.92) .. (539.73,313.65) .. controls (539.73,317.38) and (535.45,320.41) .. (530.18,320.41) .. controls (524.9,320.41) and (520.63,317.38) .. (520.63,313.65) -- cycle ;
%Straight Lines [id:da3781371432487448] 
\draw    (467.69,167.92) -- (518.34,307.76) -- (519.91,311.79) ;
\draw [shift={(520.63,313.65)}, rotate = 248.82] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da09264197892508252] 
\draw    (547.77,308.9) .. controls (537.5,308.9) and (529.99,322.58) .. (568.21,313.89) ;
\draw [shift={(569.99,313.48)}, rotate = 166.67] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (197.38,228.16) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}2};
% Text Node
\draw (197.53,254) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}3};
% Text Node
\draw (198.25,176.08) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {0};
% Text Node
\draw (196.82,201.92) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}1};
% Text Node
\draw (212.86,195.68) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (212.86,279.04) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (197.53,281.01) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}4};
% Text Node
\draw (197.53,313.43) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}5};
% Text Node
\draw (198.97,147.52) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {1};
% Text Node
\draw (182.93,179.47) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (229.25,201.85) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \nu $};
% Text Node
\draw (399.27,223.46) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}2};
% Text Node
\draw (399.42,249.3) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}3};
% Text Node
\draw (400.15,171.38) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {0};
% Text Node
\draw (398.71,197.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}1};
% Text Node
\draw (414.75,190.98) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (414.75,274.33) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (399.42,276.31) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}4};
% Text Node
\draw (399.42,308.73) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}5};
% Text Node
\draw (400.86,142.82) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {1};
% Text Node
\draw (384.82,174.77) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (431.14,197.15) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \nu $};
% Text Node
\draw (572.73,223.46) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}2};
% Text Node
\draw (572.88,249.3) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}3};
% Text Node
\draw (573.6,171.38) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {0};
% Text Node
\draw (572.17,197.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}1};
% Text Node
\draw (588.21,190.98) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (588.21,274.33) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (572.88,276.31) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}4};
% Text Node
\draw (572.88,308.73) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {\mbox{-}5};
% Text Node
\draw (574.32,142.82) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.6 ] [align=left] {1};
% Text Node
\draw (558.28,174.77) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \eta $};
% Text Node
\draw (604.6,197.15) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.8 ] [align=left] {$\displaystyle \nu $};
% Text Node
\draw (104.17,168.29) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \eta ^{2}$};
% Text Node
\draw (249.86,230.88) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (312.21,195.12) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \eta \nu $};
% Text Node
\draw (449.85,237.46) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (497.06,235.52) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \nu ^{2}$};


\end{tikzpicture}
\]
which means $\eta^2[-1]=\nu^2[-5]$. Therefore we know $N=5$ and $M(\eta^2)=\nu^2$.

\subsection{$M(\nu)$}
Since homotopy groups $\pi_4$ and $\pi_5$ are trivial, we know $N\geq4$. By proposition 4.4, there is an attaching map $\nu$ from 0-cell to $-4$-cell, so $\nu^2[-4]$ is killed by $\nu[0]$ through $d_4$ differential and we know $|M(\nu)|\neq6$ and $N\geq5$.

When $N=5$, we compute the AHSS of $P^{\infty}_{-5}$ to find that $\sigma[-5]$ survives in the $E_{\infty}$ page and $2\sigma[-5]$ is killed by $\sigma[-4]$ through $d_1$ differential. So $\sigma[-5]$ is a generator of $\pi_2(P^{\infty}_{-5})$. We can also deduce that $\nu[-1]=\sigma[-5]$ by the similar discussion as in the case ``$\eta$". Therefore, we know $N=5$ and $M(\nu)=\sigma+\langle2\sigma\rangle$.

\begin{remark}
    If we compute $\pi_2(P^{\infty}_{-5})$ by the AHSS, we will find that $\nu^2[-4]$ will survive in the $E_{\infty}$ page because $\nu[0]$ can't survive in the $E_1$ page although there is an attaching map $\nu$ from 0-cell to $-4$-cell. However we have $\pi_2(P^{\infty}_{-5})=\Z_2\{\sigma[-5]\}$ in fact because there is a hidden extension before the Atiyah-Hirzebruch differential: $\eta[-2]=\nu[-4]$ and $\eta[2]$ survives in the $E_4$ page.
    So we have:
    \[
    d_4(\eta[-2])=\nu\cdot\eta[-2]=\nu^2[-4]
    \]
    and $\nu^2[-4]$ is not a generator of $\pi_2(P^{\infty}_{-5})$.
\end{remark}








The computations of $\pi_k(P^{\infty}_{-N})$ by the AHSS and extensions in the cell diagrams will be very complicated when the stems are relatively high, so this method has some limitations. Behrens presents Mahowald invariants of elements whose stems are below 14 other than $\epsilon$ and $\eta\epsilon$ by two other methods in [], where he applies the filtration of elements to simplify the computations. 




\subsection{Toda bracket}

\begin{lemma}
Suppose $\alpha\cdot\beta=0$, then we have\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Circle [id:dp540435629244747] 
\draw   (101,214.67) .. controls (101,211.17) and (103.84,208.33) .. (107.33,208.33) .. controls (110.83,208.33) and (113.67,211.17) .. (113.67,214.67) .. controls (113.67,218.16) and (110.83,221) .. (107.33,221) .. controls (103.84,221) and (101,218.16) .. (101,214.67) -- cycle ;
%Shape: Circle [id:dp8639632606629888] 
\draw   (101,253.67) .. controls (101,250.17) and (103.84,247.33) .. (107.33,247.33) .. controls (110.83,247.33) and (113.67,250.17) .. (113.67,253.67) .. controls (113.67,257.16) and (110.83,260) .. (107.33,260) .. controls (103.84,260) and (101,257.16) .. (101,253.67) -- cycle ;
%Straight Lines [id:da11578215356481447] 
\draw    (107.33,221) -- (107.33,247.33) ;
%Shape: Circle [id:dp6831199725178945] 
\draw   (190,214.67) .. controls (190,211.17) and (192.84,208.33) .. (196.33,208.33) .. controls (199.83,208.33) and (202.67,211.17) .. (202.67,214.67) .. controls (202.67,218.16) and (199.83,221) .. (196.33,221) .. controls (192.84,221) and (190,218.16) .. (190,214.67) -- cycle ;
%Shape: Circle [id:dp52394495931562] 
\draw   (190,253.67) .. controls (190,250.17) and (192.84,247.33) .. (196.33,247.33) .. controls (199.83,247.33) and (202.67,250.17) .. (202.67,253.67) .. controls (202.67,257.16) and (199.83,260) .. (196.33,260) .. controls (192.84,260) and (190,257.16) .. (190,253.67) -- cycle ;
%Straight Lines [id:da0771608627427911] 
\draw    (196.33,221) -- (196.33,247.33) ;
%Straight Lines [id:da5866183597375858] 
\draw    (113.67,214.67) -- (148,214.33) ;
\draw [shift={(148,214.33)}, rotate = 179.44] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (17.64,-4.9) .. controls (13.66,-2.3) and (10.02,-0.67) .. (6.71,0) .. controls (10.02,0.67) and (13.66,2.3) .. (17.64,4.9)(10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Shape: Circle [id:dp021971773497480918] 
\draw   (148,214.33) .. controls (148,210.84) and (150.84,208) .. (154.33,208) .. controls (157.83,208) and (160.67,210.84) .. (160.67,214.33) .. controls (160.67,217.83) and (157.83,220.67) .. (154.33,220.67) .. controls (150.84,220.67) and (148,217.83) .. (148,214.33) -- cycle ;
%Straight Lines [id:da09483465901464427] 
\draw    (160.67,214.33) -- (188,214.64) ;
\draw [shift={(190,214.67)}, rotate = 180.65] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp8500375362825912] 
\draw   (239,214.67) .. controls (239,211.17) and (241.84,208.33) .. (245.33,208.33) .. controls (248.83,208.33) and (251.67,211.17) .. (251.67,214.67) .. controls (251.67,218.16) and (248.83,221) .. (245.33,221) .. controls (241.84,221) and (239,218.16) .. (239,214.67) -- cycle ;
%Shape: Circle [id:dp1308655979421567] 
\draw   (239,253.67) .. controls (239,250.17) and (241.84,247.33) .. (245.33,247.33) .. controls (248.83,247.33) and (251.67,250.17) .. (251.67,253.67) .. controls (251.67,257.16) and (248.83,260) .. (245.33,260) .. controls (241.84,260) and (239,257.16) .. (239,253.67) -- cycle ;
%Straight Lines [id:da2898232574475539] 
\draw    (245.33,221) -- (245.33,247.33) ;
%Shape: Circle [id:dp08539098428019676] 
\draw   (352,214.67) .. controls (352,211.17) and (354.84,208.33) .. (358.33,208.33) .. controls (361.83,208.33) and (364.67,211.17) .. (364.67,214.67) .. controls (364.67,218.16) and (361.83,221) .. (358.33,221) .. controls (354.84,221) and (352,218.16) .. (352,214.67) -- cycle ;
%Shape: Circle [id:dp8274906334622147] 
\draw   (352,253.67) .. controls (352,250.17) and (354.84,247.33) .. (358.33,247.33) .. controls (361.83,247.33) and (364.67,250.17) .. (364.67,253.67) .. controls (364.67,257.16) and (361.83,260) .. (358.33,260) .. controls (354.84,260) and (352,257.16) .. (352,253.67) -- cycle ;
%Straight Lines [id:da4664883247494891] 
\draw    (358.33,221) -- (358.33,247.33) ;
%Shape: Circle [id:dp6556369433510494] 
\draw   (286,254.33) .. controls (286,250.84) and (288.84,248) .. (292.33,248) .. controls (295.83,248) and (298.67,250.84) .. (298.67,254.33) .. controls (298.67,257.83) and (295.83,260.67) .. (292.33,260.67) .. controls (288.84,260.67) and (286,257.83) .. (286,254.33) -- cycle ;
%Straight Lines [id:da7691911446689081] 
\draw    (251.67,253.67) -- (284,254.29) ;
\draw [shift={(286,254.33)}, rotate = 181.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8090763857124177] 
\draw    (298.67,254.33) -- (350,253.69) ;
\draw [shift={(352,253.67)}, rotate = 179.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (98,229) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (169,203) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (198.33,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (215,225) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (236,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (360.33,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (262.33,244) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};


\end{tikzpicture}
\]  
\end{lemma}
\begin{proof}
By the definition of the map to a cell diagram, the indeterminacy of the two sides of the equality are the same:c

Consider the induced long exact homotopy groups associated to the following diagram:\[
\begin{tikzcd}
                                         & S^{|\alpha|} \arrow[r, "\alpha"]                                 & S^0 \arrow[r, "i"]                           & C\alpha \arrow[r, "p"]                                            & S^{|\alpha|+1} \arrow[r, "\alpha"]                  & S^1 \\
S^{|\alpha |+|\beta|} \arrow[r, "\beta"] & S^{|\alpha|} \arrow[r, "i"] \arrow[u, "id", no head, Rightarrow] & C\beta \arrow[r, "p"] \arrow[u, "f", dashed] & S^{|\alpha |+|\beta|+1} \arrow[r, "\beta"] \arrow[u, "g", dashed] & S^{|\alpha|+1} \arrow[u, "id", no head, Rightarrow] &    
\end{tikzcd}
\],
and we choose $f$ and $g$ such that the first square and the third square commutes. Since $p\circ i=0$ and $p\circ g\circ p=\beta\circ p=0$, we obtain $i\circ f-g\circ p\in \ker p_*=\im i_*$, which means there exists $h:C\beta\rightarrow S^0$ such that $i\circ f-g\circ p=i\circ h$. So the second square commutes up to the indeterminacy
\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Circle [id:dp8500375362825912] 
\draw   (194,214.67) .. controls (194,211.17) and (196.84,208.33) .. (200.33,208.33) .. controls (203.83,208.33) and (206.67,211.17) .. (206.67,214.67) .. controls (206.67,218.16) and (203.83,221) .. (200.33,221) .. controls (196.84,221) and (194,218.16) .. (194,214.67) -- cycle ;
%Shape: Circle [id:dp1308655979421567] 
\draw   (194,253.67) .. controls (194,250.17) and (196.84,247.33) .. (200.33,247.33) .. controls (203.83,247.33) and (206.67,250.17) .. (206.67,253.67) .. controls (206.67,257.16) and (203.83,260) .. (200.33,260) .. controls (196.84,260) and (194,257.16) .. (194,253.67) -- cycle ;
%Straight Lines [id:da2898232574475539] 
\draw    (200.33,221) -- (200.33,247.33) ;
%Shape: Circle [id:dp08539098428019676] 
\draw   (352,214.67) .. controls (352,211.17) and (354.84,208.33) .. (358.33,208.33) .. controls (361.83,208.33) and (364.67,211.17) .. (364.67,214.67) .. controls (364.67,218.16) and (361.83,221) .. (358.33,221) .. controls (354.84,221) and (352,218.16) .. (352,214.67) -- cycle ;
%Shape: Circle [id:dp8274906334622147] 
\draw   (352,253.67) .. controls (352,250.17) and (354.84,247.33) .. (358.33,247.33) .. controls (361.83,247.33) and (364.67,250.17) .. (364.67,253.67) .. controls (364.67,257.16) and (361.83,260) .. (358.33,260) .. controls (354.84,260) and (352,257.16) .. (352,253.67) -- cycle ;
%Straight Lines [id:da4664883247494891] 
\draw    (358.33,221) -- (358.33,247.33) ;
%Shape: Circle [id:dp6556369433510494] 
\draw   (286,254.33) .. controls (286,250.84) and (288.84,248) .. (292.33,248) .. controls (295.83,248) and (298.67,250.84) .. (298.67,254.33) .. controls (298.67,257.83) and (295.83,260.67) .. (292.33,260.67) .. controls (288.84,260.67) and (286,257.83) .. (286,254.33) -- cycle ;
%Straight Lines [id:da8090763857124177] 
\draw    (298.67,254.33) -- (350,253.69) ;
\draw [shift={(352,253.67)}, rotate = 179.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp6978983712674935] 
\draw   (247,214.33) .. controls (247,210.84) and (249.84,208) .. (253.33,208) .. controls (256.83,208) and (259.67,210.84) .. (259.67,214.33) .. controls (259.67,217.83) and (256.83,220.67) .. (253.33,220.67) .. controls (249.84,220.67) and (247,217.83) .. (247,214.33) -- cycle ;
%Straight Lines [id:da6277334276338764] 
\draw    (206.67,214.67) -- (247,214.33) ;
\draw [shift={(247,214.33)}, rotate = 179.53] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (17.64,-4.9) .. controls (13.66,-2.3) and (10.02,-0.67) .. (6.71,0) .. controls (10.02,0.67) and (13.66,2.3) .. (17.64,4.9)(10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Straight Lines [id:da9345188607731334] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (259.67,214.33) -- (284.9,252.66) ;
\draw [shift={(286,254.33)}, rotate = 236.64] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (191,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (360.33,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};


\end{tikzpicture}
\]
Since the elements of the left side of the equality are the form $g\circ p$ and the elements of the right side of the equality are the form $i\circ f$, we prove the lemma.
\end{proof}

\begin{corollary}
If $\alpha\cdot\beta=0$ and $\beta\cdot\gamma=0$,then\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Circle [id:dp8500375362825912] 
\draw   (165,214.67) .. controls (165,211.17) and (167.84,208.33) .. (171.33,208.33) .. controls (174.83,208.33) and (177.67,211.17) .. (177.67,214.67) .. controls (177.67,218.16) and (174.83,221) .. (171.33,221) .. controls (167.84,221) and (165,218.16) .. (165,214.67) -- cycle ;
%Shape: Circle [id:dp1308655979421567] 
\draw   (165,253.67) .. controls (165,250.17) and (167.84,247.33) .. (171.33,247.33) .. controls (174.83,247.33) and (177.67,250.17) .. (177.67,253.67) .. controls (177.67,257.16) and (174.83,260) .. (171.33,260) .. controls (167.84,260) and (165,257.16) .. (165,253.67) -- cycle ;
%Straight Lines [id:da2898232574475539] 
\draw    (171.33,221) -- (171.33,247.33) ;
%Shape: Circle [id:dp08539098428019676] 
\draw   (276,214.67) .. controls (276,211.17) and (278.84,208.33) .. (282.33,208.33) .. controls (285.83,208.33) and (288.67,211.17) .. (288.67,214.67) .. controls (288.67,218.16) and (285.83,221) .. (282.33,221) .. controls (278.84,221) and (276,218.16) .. (276,214.67) -- cycle ;
%Shape: Circle [id:dp8274906334622147] 
\draw   (276,253.67) .. controls (276,250.17) and (278.84,247.33) .. (282.33,247.33) .. controls (285.83,247.33) and (288.67,250.17) .. (288.67,253.67) .. controls (288.67,257.16) and (285.83,260) .. (282.33,260) .. controls (278.84,260) and (276,257.16) .. (276,253.67) -- cycle ;
%Straight Lines [id:da4664883247494891] 
\draw    (282.33,221) -- (282.33,247.33) ;
%Shape: Circle [id:dp6556369433510494] 
\draw   (210,254.33) .. controls (210,250.84) and (212.84,248) .. (216.33,248) .. controls (219.83,248) and (222.67,250.84) .. (222.67,254.33) .. controls (222.67,257.83) and (219.83,260.67) .. (216.33,260.67) .. controls (212.84,260.67) and (210,257.83) .. (210,254.33) -- cycle ;
%Straight Lines [id:da8090763857124177] 
\draw    (222.67,254.33) -- (274,253.69) ;
\draw [shift={(276,253.67)}, rotate = 179.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp6978983712674935] 
\draw   (114,214.33) .. controls (114,210.84) and (116.84,208) .. (120.33,208) .. controls (123.83,208) and (126.67,210.84) .. (126.67,214.33) .. controls (126.67,217.83) and (123.83,220.67) .. (120.33,220.67) .. controls (116.84,220.67) and (114,217.83) .. (114,214.33) -- cycle ;
%Straight Lines [id:da09530737044541926] 
\draw    (126.67,214.33) -- (163,214.65) ;
\draw [shift={(165,214.67)}, rotate = 180.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3119861017557841] 
\draw    (177.67,253.67) -- (208,254.29) ;
\draw [shift={(210,254.33)}, rotate = 181.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp3321637436628957] 
\draw   (385,215.67) .. controls (385,212.17) and (387.84,209.33) .. (391.33,209.33) .. controls (394.83,209.33) and (397.67,212.17) .. (397.67,215.67) .. controls (397.67,219.16) and (394.83,222) .. (391.33,222) .. controls (387.84,222) and (385,219.16) .. (385,215.67) -- cycle ;
%Shape: Circle [id:dp3559801028823957] 
\draw   (439,215.67) .. controls (439,212.17) and (441.84,209.33) .. (445.33,209.33) .. controls (448.83,209.33) and (451.67,212.17) .. (451.67,215.67) .. controls (451.67,219.16) and (448.83,222) .. (445.33,222) .. controls (441.84,222) and (439,219.16) .. (439,215.67) -- cycle ;
%Shape: Circle [id:dp40342052690731545] 
\draw   (439,254.67) .. controls (439,251.17) and (441.84,248.33) .. (445.33,248.33) .. controls (448.83,248.33) and (451.67,251.17) .. (451.67,254.67) .. controls (451.67,258.16) and (448.83,261) .. (445.33,261) .. controls (441.84,261) and (439,258.16) .. (439,254.67) -- cycle ;
%Straight Lines [id:da5175438784550372] 
\draw    (445.33,222) -- (445.33,248.33) ;
%Shape: Circle [id:dp11717752529634873] 
\draw   (334,215.33) .. controls (334,211.84) and (336.84,209) .. (340.33,209) .. controls (343.83,209) and (346.67,211.84) .. (346.67,215.33) .. controls (346.67,218.83) and (343.83,221.67) .. (340.33,221.67) .. controls (336.84,221.67) and (334,218.83) .. (334,215.33) -- cycle ;
%Straight Lines [id:da8306476893360741] 
\draw    (346.67,215.33) -- (383,215.65) ;
\draw [shift={(385,215.67)}, rotate = 180.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da17091831315888784] 
\draw    (397.67,215.67) -- (437,215.67) ;
\draw [shift={(439,215.67)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (162,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (284.33,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (187.33,243) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (141.33,205) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (140.67,204.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \gamma $};
% Text Node
\draw (302,226) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (447.33,229) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (361.33,206) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (360.67,205.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \gamma $};
% Text Node
\draw (410.67,204.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (412.67,205.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};


\end{tikzpicture}
\]
\end{corollary}
\begin{proof}
By Lemma 7.3, we have\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Circle [id:dp8500375362825912] 
\draw   (114,214.67) .. controls (114,211.17) and (116.84,208.33) .. (120.33,208.33) .. controls (123.83,208.33) and (126.67,211.17) .. (126.67,214.67) .. controls (126.67,218.16) and (123.83,221) .. (120.33,221) .. controls (116.84,221) and (114,218.16) .. (114,214.67) -- cycle ;
%Shape: Circle [id:dp1308655979421567] 
\draw   (114,253.67) .. controls (114,250.17) and (116.84,247.33) .. (120.33,247.33) .. controls (123.83,247.33) and (126.67,250.17) .. (126.67,253.67) .. controls (126.67,257.16) and (123.83,260) .. (120.33,260) .. controls (116.84,260) and (114,257.16) .. (114,253.67) -- cycle ;
%Straight Lines [id:da2898232574475539] 
\draw    (120.33,221) -- (120.33,247.33) ;
%Shape: Circle [id:dp08539098428019676] 
\draw   (202,215.67) .. controls (202,212.17) and (204.84,209.33) .. (208.33,209.33) .. controls (211.83,209.33) and (214.67,212.17) .. (214.67,215.67) .. controls (214.67,219.16) and (211.83,222) .. (208.33,222) .. controls (204.84,222) and (202,219.16) .. (202,215.67) -- cycle ;
%Shape: Circle [id:dp8274906334622147] 
\draw   (202,254.67) .. controls (202,251.17) and (204.84,248.33) .. (208.33,248.33) .. controls (211.83,248.33) and (214.67,251.17) .. (214.67,254.67) .. controls (214.67,258.16) and (211.83,261) .. (208.33,261) .. controls (204.84,261) and (202,258.16) .. (202,254.67) -- cycle ;
%Straight Lines [id:da4664883247494891] 
\draw    (208.33,222) -- (208.33,248.33) ;
%Shape: Circle [id:dp6556369433510494] 
\draw   (159,254.33) .. controls (159,250.84) and (161.84,248) .. (165.33,248) .. controls (168.83,248) and (171.67,250.84) .. (171.67,254.33) .. controls (171.67,257.83) and (168.83,260.67) .. (165.33,260.67) .. controls (161.84,260.67) and (159,257.83) .. (159,254.33) -- cycle ;
%Shape: Circle [id:dp6978983712674935] 
\draw   (63,214.33) .. controls (63,210.84) and (65.84,208) .. (69.33,208) .. controls (72.83,208) and (75.67,210.84) .. (75.67,214.33) .. controls (75.67,217.83) and (72.83,220.67) .. (69.33,220.67) .. controls (65.84,220.67) and (63,217.83) .. (63,214.33) -- cycle ;
%Straight Lines [id:da09530737044541926] 
\draw    (75.67,214.33) -- (112,214.65) ;
\draw [shift={(114,214.67)}, rotate = 180.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3119861017557841] 
\draw    (126.67,253.67) -- (157,254.29) ;
\draw [shift={(159,254.33)}, rotate = 181.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp3321637436628957] 
\draw   (495,215.67) .. controls (495,212.17) and (497.84,209.33) .. (501.33,209.33) .. controls (504.83,209.33) and (507.67,212.17) .. (507.67,215.67) .. controls (507.67,219.16) and (504.83,222) .. (501.33,222) .. controls (497.84,222) and (495,219.16) .. (495,215.67) -- cycle ;
%Shape: Circle [id:dp3559801028823957] 
\draw   (549,215.67) .. controls (549,212.17) and (551.84,209.33) .. (555.33,209.33) .. controls (558.83,209.33) and (561.67,212.17) .. (561.67,215.67) .. controls (561.67,219.16) and (558.83,222) .. (555.33,222) .. controls (551.84,222) and (549,219.16) .. (549,215.67) -- cycle ;
%Shape: Circle [id:dp40342052690731545] 
\draw   (549,254.67) .. controls (549,251.17) and (551.84,248.33) .. (555.33,248.33) .. controls (558.83,248.33) and (561.67,251.17) .. (561.67,254.67) .. controls (561.67,258.16) and (558.83,261) .. (555.33,261) .. controls (551.84,261) and (549,258.16) .. (549,254.67) -- cycle ;
%Straight Lines [id:da5175438784550372] 
\draw    (555.33,222) -- (555.33,248.33) ;
%Shape: Circle [id:dp11717752529634873] 
\draw   (444,215.33) .. controls (444,211.84) and (446.84,209) .. (450.33,209) .. controls (453.83,209) and (456.67,211.84) .. (456.67,215.33) .. controls (456.67,218.83) and (453.83,221.67) .. (450.33,221.67) .. controls (446.84,221.67) and (444,218.83) .. (444,215.33) -- cycle ;
%Straight Lines [id:da8306476893360741] 
\draw    (456.67,215.33) -- (493,215.65) ;
\draw [shift={(495,215.67)}, rotate = 180.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da17091831315888784] 
\draw    (507.67,215.67) -- (547,215.67) ;
\draw [shift={(549,215.67)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6302920227588535] 
\draw    (171.67,254.33) -- (200,254.64) ;
\draw [shift={(202,254.67)}, rotate = 180.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp07282200238501146] 
\draw   (292,215.67) .. controls (292,212.17) and (294.84,209.33) .. (298.33,209.33) .. controls (301.83,209.33) and (304.67,212.17) .. (304.67,215.67) .. controls (304.67,219.16) and (301.83,222) .. (298.33,222) .. controls (294.84,222) and (292,219.16) .. (292,215.67) -- cycle ;
%Shape: Circle [id:dp37124668587600596] 
\draw   (292,254.67) .. controls (292,251.17) and (294.84,248.33) .. (298.33,248.33) .. controls (301.83,248.33) and (304.67,251.17) .. (304.67,254.67) .. controls (304.67,258.16) and (301.83,261) .. (298.33,261) .. controls (294.84,261) and (292,258.16) .. (292,254.67) -- cycle ;
%Straight Lines [id:da4839232363695676] 
\draw    (298.33,222) -- (298.33,248.33) ;
%Shape: Circle [id:dp19999996938989661] 
\draw   (245,216.33) .. controls (245,212.84) and (247.84,210) .. (251.33,210) .. controls (254.83,210) and (257.67,212.84) .. (257.67,216.33) .. controls (257.67,219.83) and (254.83,222.67) .. (251.33,222.67) .. controls (247.84,222.67) and (245,219.83) .. (245,216.33) -- cycle ;
%Straight Lines [id:da6880920476429031] 
\draw    (257.67,216.33) -- (290,215.71) ;
\draw [shift={(292,215.67)}, rotate = 178.89] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp21609833961440317] 
\draw   (337,215.67) .. controls (337,212.17) and (339.84,209.33) .. (343.33,209.33) .. controls (346.83,209.33) and (349.67,212.17) .. (349.67,215.67) .. controls (349.67,219.16) and (346.83,222) .. (343.33,222) .. controls (339.84,222) and (337,219.16) .. (337,215.67) -- cycle ;
%Shape: Circle [id:dp160626954549691] 
\draw   (391,215.67) .. controls (391,212.17) and (393.84,209.33) .. (397.33,209.33) .. controls (400.83,209.33) and (403.67,212.17) .. (403.67,215.67) .. controls (403.67,219.16) and (400.83,222) .. (397.33,222) .. controls (393.84,222) and (391,219.16) .. (391,215.67) -- cycle ;
%Shape: Circle [id:dp9529004011959146] 
\draw   (391,254.67) .. controls (391,251.17) and (393.84,248.33) .. (397.33,248.33) .. controls (400.83,248.33) and (403.67,251.17) .. (403.67,254.67) .. controls (403.67,258.16) and (400.83,261) .. (397.33,261) .. controls (393.84,261) and (391,258.16) .. (391,254.67) -- cycle ;
%Straight Lines [id:da21178828777955738] 
\draw    (397.33,222) -- (397.33,248.33) ;
%Straight Lines [id:da7079732944172863] 
\draw    (349.67,215.67) -- (389,215.67) ;
\draw [shift={(391,215.67)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da11508840406268295] 
\draw    (304.67,215.67) -- (337,215.67) ;
\draw [shift={(337,215.67)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (17.64,-4.9) .. controls (13.66,-2.3) and (10.02,-0.67) .. (6.71,0) .. controls (10.02,0.67) and (13.66,2.3) .. (17.64,4.9)(10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;

% Text Node
\draw (111,228) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (210.33,229) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (136.33,243) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (90.33,205) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (89.67,204.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \gamma $};
% Text Node
\draw (224,226) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};
% Text Node
\draw (557.33,229) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (471.33,206) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (470.67,205.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \gamma $};
% Text Node
\draw (520.67,204.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (522.67,205.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (289,229) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (272.33,207) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (271.67,206.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \gamma $};
% Text Node
\draw (399.33,229) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (362.67,204.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$ $};
% Text Node
\draw (364.67,205.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \beta $};
% Text Node
\draw (419,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {=};


\end{tikzpicture}
\]
\end{proof}

\subsection{results}
\begin{basedescript}{\desclabelstyle{\pushlabel}\desclabelwidth{4em}}
    \item[$R(\epsilon)$] The element $\epsilon$ is detected by $c_0$ in the ASS, and $c_1\in R_{alg}(c_0)$ with no indeterminacy. Because $c_1$ survives in the $E_{\infty}$-page and detects $\bar{\sigma}$, and $h_{\#}(c_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-12}$, by Theorem 6.4(c) we deduce that $\bar{\sigma}\in R(\epsilon)$.
    
    \item[$R(\eta\epsilon)$] The element $\eta\epsilon$ is detected by $h_1c_0$ in the ASS, and $h_2c_1\in R_{alg}(h_1c_0)$ with no indeterminacy by Corollary 6.12. Since $h_2c_1$ survives in the $E_{\infty}$-page and detects $\nu\bar{\sigma}$, and $h_{\#}(h_2c_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-14}$, by Theorem 6.4(c) we deduce that $\nu\bar{\sigma}\in R(\eta\epsilon)$.

    \item[$R(\sigma^2)$] The element $\sigma^2$ is detected by $h_3^2$ in the ASS, and $h_4^2\in R_{alg}(h_3^2)$ with no indeterminacy by Corollary 6.12.
    Since $h_4^2$ survives in the $E_{\infty}$-page and detects $\theta_4$, and $h_{\#}(h_4^2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-17}$, by Theorem 6.4(c) we deduce that $\theta_4\in R(\sigma^2)$.

    \item[$R(\kappa)$] The element $\kappa$ is detected by $d_0$ in the ASS, and $d_1\in R_{alg}(d_0)$ with no indeterminacy. Since $d_1$ survives in the $E_{\infty}$-page and detects $\kappa_1$, and $h_{\#}(d_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-19}$, by Theorem 6.4(c) we deduce that $\kappa_1\in R(\kappa)$.
    
    \item[$R(\eta\kappa)$] The element $\eta\kappa$ is detected by $h_1d_0$ in the ASS and $h_2d_1\in R_{alg}(h_1d_0)$ with no indeterminacy by Corollary 6.12. Since $h_2d_1$ survives in the $E_{\infty}$-page and detects $\nu\kappa_1$, and $h_{\#}(h_2d_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-21}$, by Theorem 6.4(c) we deduce that $\nu\kappa_1\in R(\eta\kappa)$.

    \item[$R(\rho_{15})$] The element $\rho_{15}$ is detected by $h_0^3h_4$ in the ASS. and $h_0^2h_2h_5\in R_{alg}(h_0^3h_4)$ with no indeterminacy by Corollary 6.12. Since $h_0^2h_2h_5$ survives in the $E_{\infty}$-page and detects $\eta^2\eta_5$, and $h_{\#}(h_0^2h_2h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-20}$, by Theorem 6.4(c) we deduce that $\eta^2\eta_5\in R(\rho_{15})$./

    \item[$R(2\rho_{15})$] The element $2\rho_{15}$ is detected by $h_0^4h_4$ in the ASS and $h_0^3h_3h_5\in R_{alg}(h_0^4h_4)$ with no indeterminacy by []. Since $h_0^3h_3h_5$ survives in the $E_{\infty}$-page, and $h_{\#}(h_0^3h_3h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-24}$, by Theorem 6.4(c) we deduce that $\{h_0^3h_3h_5\}\in R(2\rho_{15})$.

    \item[$R(4\rho_{15})$] The element $4\rho_{15}$ is detected by $h_0^5h_4$ in the ASS and $h_5Ph_1\in R_{alg}(h_0^5h_4)$ with indeterminacy $h_0^2f_1$. Since $\{h_5Ph_1\}$ survives in the $E_{\infty}$-page and $h_0^2f_1$ is killed by $h_0c_2$ through $d_2$ differential, and $h_{\#}(h_5Ph_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-26}$, by Theorem 6.4(c) we deduce that $\{h_5Ph_1\}\in R(4\rho_{15})$.

    \item[$R(8\rho_{15})$] The element $8\rho_{15}$ is detected by $h_0^6h_4$ in the ASS and $h_1h_5Ph_1\in R_{alg}(h_0^6h_4)$ with no indeterminacy by Corollary 6.12. Since $h_1h_5Ph_1$ survives in the $E_{\infty}$-page and detects $\eta\{h_5Ph_1\}$, and $h_{\#}(h_1h_5Ph_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-27}$, by Theorem 6.4(c) we deduce that $\eta\{h_5Ph_1\}\in R(8\rho_{15})$.

    \item[$R(16\rho_{15})$] The element $16\rho_{15}$ is detected by $h_0^7h_4$ in the ASS and $h_0^2h_5Ph_2\in R_{alg}(h_0^7h_4)$ with no indeterminacy by Corollary 6.12. Since $h_0^2h_5Ph_2$ survives in the $E_{\infty}$-page and detects $4\{h_5Ph_2\}$, and $h_{\#}(h_0^2h_5Ph_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-28}$, by Theorem 6.4(c) we deduce that $4\{h_5Ph_2\}\in R(16\rho_{15})$.

    \item[$R(\eta\rho_{15})$] The element $\eta\rho_{15}$ is detected by $Pc_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^3h_4$ to $Pc_0 $ by [0-90], and $h_1\triangle h_3^2$ (or denoted as $h_2t)\in R_{alg}(Pc_0)$ with no indeterminacy. Since $h_1\triangle h_3^2$ survives in the $E_{\infty}$-page and detects $\nu\{t\}$, and $h_{\#}(h_1\triangle h_3^2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-24}$, by Theorem 6.4(c) we deduce that $\nu\{t\}\in R(\eta\rho_{15})$.

    \item[$R(\eta\eta_4)$] The element $\eta\eta_4$ is detected by $h_1^2h_4$ in the ASS and $h_2^2h_5\in R_{alg}(h_1h_4)$ with no indeterminacy by Corollary 6.12. Since $h_2^2h_5$ survives in the $E_{\infty}$-page, and $h_{\#}(h_2^2h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-21}$, by Theorem 6.4(c) we deduce that $\{h_2^2h_5\}\in R(\eta\eta_4)$.

    \item[$R(\eta^2\rho_{15})$] The element $\eta^2\rho_{15}$ is detected by $h_1Pc_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^3h_4$ to $Pc_0 $ by [0-90], and $\triangle h_2c_1$ (or denoted as $N)\in R_{alg}(h_1Pc_0)$ with no indeterminacy. Since $\triangle h_2c_1$ survives in the $E_{\infty}$-page and there is a hidden $\eta$-extension from $\eta\bar{\kappa}_2$ to $\{\triangle h_2c_1\}$ by [0-90], and $h_{\#}(\triangle h_2c_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-30}$, by Theorem 6.4(c) we deduce we deduce that $\eta^2\bar{\kappa}_2\in R(\eta^2\rho_{15})$.

    \item[$R(\nu\kappa)$] The element $\nu\kappa$ is detected by $h_2d_0$ in the ASS, and $h_3d_1\in R_{alg}(h_2d_0)$ with no indeterminacy by Corollary 6.12. Since $h_3d_1$ survives in the $E_{\infty}$-page and detects $\sigma\kappa_1$, and $h_{\#}(h_3d_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-23}$, by Theorem 6.4(c) we deduce that $\sigma\kappa_1\in R(\nu\kappa)$.

    \item[$R(\mu_{17})$] The element $\mu_{17}$ is detected by $P^2h_1$ in the ASS, and $h_1h_5Pc_0\in R_{alg}(P^2h_1)$ with no indeterminacy. Since $h_1Ph_5c_0$ survives in the $E_{\infty}$-page and detects $\eta\{Ph_5c_0\}$, and $h_{\#}(h_1h_5Pc_0)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-32}$, by Theorem 6.4(c) we deduce that $\eta\{Ph_5c_0\}\in R(\mu_{17})$.

    \item[$R(2\nu_4)$] The element $2\nu_4$ is detected by $h_0h_2h_4$ in the ASS, and by Corollary 6.12 $h_1h_3h_5\in R_{alg}(h_0h_2h_4)$ with no indeterminacy. Since $h_1h_3h_5$ survives in the $E_{\infty}$-page and detects $\sigma\eta_5$, and $h_{\#}(h_1h_3h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-22}$, by Theorem 6.4(c) we deduce that $\sigma\eta_5\in R(2\nu_4)$.

    \item[$R(4\nu_4)$] The element $4\nu_4$ is detected by $h_0^2h_2h_4$ in the ASS, and by Corollary 6.12 $h_1^2h_3h_5\in R_{alg}(h_0^2h_2h_4)$ with no indeterminacy . Since $h_1^2h_3h_5$ survives in the $E_{\infty}$-page and detects $\sigma^2\eta_5$, and $h_{\#}(h_1^2h_3h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-23}$, by Theorem 6.4(c) we deduce that $\sigma^2\eta_5\in R(4\nu_4)$.

    \item [$R(\bar{\kappa})$] The element $\bar{\kappa}4$ is detected by $g$ in the ASS, and $g_2\in R_{alg}(g)$ with no indeterminacy. Since $g_2$ survives in the $E_{\infty}$-page and detects $\bar{\kappa}_2$, and $h_{\#}(g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-25}$, by Theorem 6.4(c) we deduce that $\bar{\kappa}_2\in R(\bar{\kappa})$.

     \item [$R(2\bar{\kappa})$] The element $2\bar{\kappa}4$ is detected by $h_0g$ in the ASS, and by Corollary 6.12 $h_1g_2\in R_{alg}(h_0g)$ with no indeterminacy. Since $h_1g_2$ survives in the $E_{\infty}$-page and detects $\eta\bar{\kappa}_2$, and $h_{\#}(h_1g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-26}$, by Theorem 6.4(c) we deduce that $\eta\bar{\kappa}_2\in R(\bar{2\kappa})$.

     \item[$R(\eta\bar{\kappa})$] The element $\eta\bar{\kappa}$ is detected by $h_1g$ in the ASS, and by Corollary 6.12 $h_2g_2\in R_{alg}(h_1g)$ with no indeterminacy. Since $h_2g_2$ survives in the $E_{\infty}$-page and detects $\nu\bar{\kappa}_2$, and $h_{\#}(h_2g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-27}$, by Theorem 6.4(c) we deduce that $\nu\bar{\kappa}_2\in R(\eta\bar{\kappa})$.

      \item[$R(\nu\nu_4)$] The element $\nu\nu_4=\sigma^3$ is detected by $h_2^2h_4$ in the ASS, and by Corollary 6.12 $h_3^2h_5=h_4^3\in R_{alg}(h_2^2h_4)$ with no indeterminacy. Since $h_3^2h_5$ survives in the $E_{\infty}$-page and detects $\theta_{4,5}$, and $h_{\#}(h_3^2h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-25}$, by Theorem 6.4(c) we deduce that $\theta_{4,5}\in R(\nu\nu_4)$.

     \item[$R(\eta^2\bar{\kappa})$] The element $\eta^2\kappa$ is detected by $Pd_0$ in the ASS because there is a  hidden $\eta$-extension from $\eta\bar{\kappa}$ to $\{Pd_0\}$, and $gd_1\in R_{alg}(Pd_0)$ with no indeterminacy. Since $gd_1$ survives in the $E_{\infty}$-page and detects $\bar{\kappa}\kappa_1$, and $h_{\#}(gd_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-31}$, by Theorem 6.4(c) we deduce that $\bar{\kappa}\kappa_1\in R(\eta^2\bar{\kappa})$.

     \item[$R(\sigma\eta_4)$] The element $\sigma\eta_4$ is detected by $h_4c_0$ in the ASS because there is a  hidden $\sigma$-extension from $h_1h_4$ to $h_4c_0$, and by Corollary 6.12 $h_5c_1\in R_{alg}(h_4c_0)$ with no indeterminacy. Since $h_5c_1$ survives in the $E_{\infty}$-page and $h_{\#}(h_5c_1 )$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-28}$, by Theorem 6.4(c) we deduce that $\{h_5c_1\}\in R(\sigma\eta_4)$.

     \item[$R(\nu\bar{\kappa})$] The element $\nu\bar{\kappa}$ is detected by $h_2g$ in the ASS, and by Corollary 6.12 $h_3g_2\in R_{alg}(h_2g)$ with no indeterminacy. Since $h_3g_2$ survives in the $E_{\infty}$-page and detects $\sigma\bar{\kappa}_2$, and $h_{\#}(h_3g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-29}$ , by Theorem 6.4(c) we deduce that $\sigma\bar{\kappa}_2\in R(\nu\bar{\kappa})$.

     \item[$R(2\nu\bar{\kappa})$] The element $2\nu\bar{\kappa}$ is detected by $h_0h_2g$ in the ASS, and by Corollary 6.12 $h_1h_3g_2\in R_{alg}(h_0h_2g)$ with no indeterminacy. Since $h_1h_3g_2$ survives in the $E_{\infty}$-page and detects $\eta\sigma\bar{\kappa}_2$, and $h_{\#}(h_1h_3g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-30}$ , by Theorem 6.4(c) we deduce that $\eta\sigma\bar{\kappa}_2\in R(2\nu\bar{\kappa})$.

     \item[$R(2\rho_{23})$] The element $2\rho_{23}$ is detected by $h_0^3i$ in the ASS, and $\triangle^2h_1h_4\in R_{alg}(h_0^3i)$ with indeterminacy $h_0^2h_3Q_2$. Because $\triangle^2h_1h_4$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-42}$, by Theorem 6.4(c) we deduce that $\{\triangle^2h_1h_4\}\in R(2\rho_{23})$.
     
       \item[$R(4\rho_{23})$] The element $4\rho_{23}$ is detected by $h_0^4i$ in the ASS, and $h_1\triangle^2h_1h_4\in R_{alg}(h_0^4i)$ with indeterminacy $h_0Mg$. Because $h_1\triangle^2h_1h_4$ survives in the $E_{\infty}$-page and $h_{\#}(h_1\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-43}$, by Theorem 6.4(c) we deduce that $\eta\{\triangle^2h_1h_4\}\in R(4\rho_{23})$.
     
      \item[$R(8\rho_{23})$] The element $8\rho_{23}$ is detected by $h_0^5i$ in the ASS, and $h_1^2\triangle^2h_1h_4\in R_{alg}(h_0^5i)$ with no indeterminacy. Because $h_1^2\triangle^2h_1h_4$ survives in the $E_{\infty}$-page and $h_{\#}(h_1^2\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-44}$, by Theorem 6.4(c) we deduce that $\eta^2\{\triangle^2h_1h_4\}\in R(8\rho_{23})$.

      \item[$R(\eta\sigma\eta_4)$] The element $\eta\sigma\eta_4$ is detected by $h_1h_4c_0$ in the ASS and by Corollary 6.12 $h_2h_5c_1\in R_{alg}(h_1h_4c_0)$ with no indeterminacy. Since $h_2h_5c_1$ survives in the $E_{\infty}$-page and $h_{\#}(h_2h_5c_1 )$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-30}$, by Theorem 6.4(c) we deduce that $\nu\{h_5c_1\}\in R(\eta\sigma\eta_4)$.

      \item[$R(\eta\rho_{23})$] The element $\eta\rho_{23}$ is detected by $P^2c_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^2i$ to $P^2c_0$, and $\triangle^2c_1\in R_{alg}(P^2c_0)$ with no indeterminacy. Because $\triangle^2c_1$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-44}$, by Theorem 6.4(c) we deduce that $\{\triangle^2c_1\}\in R(\eta\rho_{23})$.
      
      \item[$R(\eta^2\rho_{23})$] The element $\eta^2\rho_{23}$ is detected by $h_1P^2c_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^2i$ to $P^2c_0$, and $h_2\triangle^2c_1\in R_{alg}(h_1P^2c_0)$ with no indeterminacy. Because $h_2\triangle^2c_1$ survives in the $E_{\infty}$-page and $h_{\#}(h_2\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-46}$, by Theorem 6.4(c) we deduce that $\nu\{\triangle^2c_1\}\in R(\eta^2\rho_{23})$.
      
      \item[$R(\mu_{25})$] The element $\mu_{25}$ is detected by $P^3h_1$ in the ASS, and $\triangle^2h_2g\in R_{alg}(P^3h_1)$ with indeterminacy $Mj$. Because $\triangle^2h_2g$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle^2h_2g)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-67}$, by Theorem 6.4(c) we deduce that $\{\triangle^2h_2g\}\in R(\mu_{25})$.

       \item[$R(\eta\mu_{25})$] The element $\eta\mu_{25}$ is detected by $h_1P^3h_1$ in the ASS, and by Corollary 6.12 $h_2\triangle^2h_2g\in R_{alg}(h_1P^3h_1)$. Because $h_2\triangle^2h_2g$ survives in the $E_{\infty}$-page and $h_{\#}(h_2\triangle^2h_2g)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-69}$, by Theorem 6.4(c) we deduce that $\nu\{\triangle^2h_2g\}\in R(\eta\mu_{25})$.

        \item[$R(\nu^2\bar{\kappa})$] The element $\nu^2\bar{\kappa}$ is detected by $h_2^2g$ in the ASS, and $\triangle_1h_3^2\in R_{alg}(h_2^2g)$ with no indeterminacy. Since $\triangle_1h_3^2$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle_1h_3^2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-41}$ , by Theorem 6.4(c) we deduce that $\{\triangle_1h_3^2\}\in R(\nu^2\bar{\kappa})$.
        
\end{basedescript}

\begin{basedescript}{\desclabelstyle{\pushlabel}\desclabelwidth{4em}}
    \item[$R(\epsilon)$] The element $\epsilon$ is detected by $c_0$ in the ASS, and $c_1\in R_{alg}(c_0)$ with no indeterminacy. Because $c_1$ survives in the $E_{\infty}$-page and detects $\bar{\sigma}$, and $h_{\#}(c_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-12}$, by Theorem 6.4(c) we deduce that $\bar{\sigma}\in R(\epsilon)$.
    
    \item[$R(\eta\epsilon)$] The element $\eta\epsilon$ is detected by $h_1c_0$ in the ASS, and $h_2c_1\in R_{alg}(h_1c_0)$ with no indeterminacy by Corollary 6.12. Since $h_2c_1$ survives in the $E_{\infty}$-page and detects $\nu\bar{\sigma}$, and $h_{\#}(h_2c_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-14}$, by Theorem 6.4(c) we deduce that $\nu\bar{\sigma}\in R(\eta\epsilon)$.

    \item[$R(\sigma^2)$] The element $\sigma^2$ is detected by $h_3^2$ in the ASS, and $h_4^2\in R_{alg}(h_3^2)$ with no indeterminacy by Corollary 6.12.
    Since $h_4^2$ survives in the $E_{\infty}$-page and detects $\theta_4$, and $h_{\#}(h_4^2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-17}$, by Theorem 6.4(c) we deduce that $\theta_4\in R(\sigma^2)$.

    \item[$R(\kappa)$] The element $\kappa$ is detected by $d_0$ in the ASS, and $d_1\in R_{alg}(d_0)$ with no indeterminacy. Since $d_1$ survives in the $E_{\infty}$-page and detects $\kappa_1$, and $h_{\#}(d_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-19}$, by Theorem 6.4(c) we deduce that $\kappa_1\in R(\kappa)$.
    
    \item[$R(\eta\kappa)$] The element $\eta\kappa$ is detected by $h_1d_0$ in the ASS and $h_2d_1\in R_{alg}(h_1d_0)$ with no indeterminacy by Corollary 6.12. Since $h_2d_1$ survives in the $E_{\infty}$-page and detects $\nu\kappa_1$, and $h_{\#}(h_2d_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-21}$, by Theorem 6.4(c) we deduce that $\nu\kappa_1\in R(\eta\kappa)$.

    \item[$R(\rho_{15})$] The element $\rho_{15}$ is detected by $h_0^3h_4$ in the ASS. and $h_0^2h_2h_5\in R_{alg}(h_0^3h_4)$ with no indeterminacy by Corollary 6.12. Since $h_0^2h_2h_5$ survives in the $E_{\infty}$-page and detects $\eta^2\eta_5$, and $h_{\#}(h_0^2h_2h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-20}$, by Theorem 6.4(c) we deduce that $\eta^2\eta_5\in R(\rho_{15})$./

    \item[$R(2\rho_{15})$] The element $2\rho_{15}$ is detected by $h_0^4h_4$ in the ASS and $h_0^3h_3h_5\in R_{alg}(h_0^4h_4)$ with no indeterminacy by []. Since $h_0^3h_3h_5$ survives in the $E_{\infty}$-page, and $h_{\#}(h_0^3h_3h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-24}$, by Theorem 6.4(c) we deduce that $\{h_0^3h_3h_5\}\in R(2\rho_{15})$.

    \item[$R(4\rho_{15})$] The element $4\rho_{15}$ is detected by $h_0^5h_4$ in the ASS and $h_5Ph_1\in R_{alg}(h_0^5h_4)$ with indeterminacy $h_0^2f_1$. Since $\{h_5Ph_1\}$ survives in the $E_{\infty}$-page and $h_0^2f_1$ is killed by $h_0c_2$ through $d_2$ differential, and $h_{\#}(h_5Ph_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-26}$, by Theorem 6.4(c) we deduce that $\{h_5Ph_1\}\in R(4\rho_{15})$.

    \item[$R(8\rho_{15})$] The element $8\rho_{15}$ is detected by $h_0^6h_4$ in the ASS and $h_1h_5Ph_1\in R_{alg}(h_0^6h_4)$ with no indeterminacy by Corollary 6.12. Since $h_1h_5Ph_1$ survives in the $E_{\infty}$-page and detects $\eta\{h_5Ph_1\}$, and $h_{\#}(h_1h_5Ph_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-27}$, by Theorem 6.4(c) we deduce that $\eta\{h_5Ph_1\}\in R(8\rho_{15})$.

    \item[$R(16\rho_{15})$] The element $16\rho_{15}$ is detected by $h_0^7h_4$ in the ASS and $h_0^2h_5Ph_2\in R_{alg}(h_0^7h_4)$ with no indeterminacy by Corollary 6.12. Since $h_0^2h_5Ph_2$ survives in the $E_{\infty}$-page and detects $4\{h_5Ph_2\}$, and $h_{\#}(h_0^2h_5Ph_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-28}$, by Theorem 6.4(c) we deduce that $4\{h_5Ph_2\}\in R(16\rho_{15})$.

    \item[$R(\eta\rho_{15})$] The element $\eta\rho_{15}$ is detected by $Pc_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^3h_4$ to $Pc_0 $ by [0-90], and $h_1\triangle h_3^2$ (or denoted as $h_2t)\in R_{alg}(Pc_0)$ with no indeterminacy. Since $h_1\triangle h_3^2$ survives in the $E_{\infty}$-page and detects $\nu\{t\}$, and $h_{\#}(h_1\triangle h_3^2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-24}$, by Theorem 6.4(c) we deduce that $\nu\{t\}\in R(\eta\rho_{15})$.

    \item[$R(\eta\eta_4)$] The element $\eta\eta_4$ is detected by $h_1^2h_4$ in the ASS and $h_2^2h_5\in R_{alg}(h_1h_4)$ with no indeterminacy by Corollary 6.12. Since $h_2^2h_5$ survives in the $E_{\infty}$-page, and $h_{\#}(h_2^2h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-21}$, by Theorem 6.4(c) we deduce that $\{h_2^2h_5\}\in R(\eta\eta_4)$.

    \item[$R(\eta^2\rho_{15})$] The element $\eta^2\rho_{15}$ is detected by $h_1Pc_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^3h_4$ to $Pc_0 $ by [0-90], and $\triangle h_2c_1$ (or denoted as $N)\in R_{alg}(h_1Pc_0)$ with no indeterminacy. Since $\triangle h_2c_1$ survives in the $E_{\infty}$-page and there is a hidden $\eta$-extension from $\eta\bar{\kappa}_2$ to $\{\triangle h_2c_1\}$ by [0-90], and $h_{\#}(\triangle h_2c_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-30}$, by Theorem 6.4(c) we deduce we deduce that $\eta^2\bar{\kappa}_2\in R(\eta^2\rho_{15})$.

    \item[$R(\nu\kappa)$] The element $\nu\kappa$ is detected by $h_2d_0$ in the ASS, and $h_3d_1\in R_{alg}(h_2d_0)$ with no indeterminacy by Corollary 6.12. Since $h_3d_1$ survives in the $E_{\infty}$-page and detects $\sigma\kappa_1$, and $h_{\#}(h_3d_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-23}$, by Theorem 6.4(c) we deduce that $\sigma\kappa_1\in R(\nu\kappa)$.

    \item[$R(\mu_{17})$] The element $\mu_{17}$ is detected by $P^2h_1$ in the ASS, and $h_1h_5Pc_0\in R_{alg}(P^2h_1)$ with no indeterminacy. Since $h_1Ph_5c_0$ survives in the $E_{\infty}$-page and detects $\eta\{Ph_5c_0\}$, and $h_{\#}(h_1h_5Pc_0)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-32}$, by Theorem 6.4(c) we deduce that $\eta\{Ph_5c_0\}\in R(\mu_{17})$.

    \item[$R(2\nu_4)$] The element $2\nu_4$ is detected by $h_0h_2h_4$ in the ASS, and by Corollary 6.12 $h_1h_3h_5\in R_{alg}(h_0h_2h_4)$ with no indeterminacy. Since $h_1h_3h_5$ survives in the $E_{\infty}$-page and detects $\sigma\eta_5$, and $h_{\#}(h_1h_3h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-22}$, by Theorem 6.4(c) we deduce that $\sigma\eta_5\in R(2\nu_4)$.

    \item[$R(4\nu_4)$] The element $4\nu_4$ is detected by $h_0^2h_2h_4$ in the ASS, and by Corollary 6.12 $h_1^2h_3h_5\in R_{alg}(h_0^2h_2h_4)$ with no indeterminacy . Since $h_1^2h_3h_5$ survives in the $E_{\infty}$-page and detects $\sigma^2\eta_5$, and $h_{\#}(h_1^2h_3h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-23}$, by Theorem 6.4(c) we deduce that $\sigma^2\eta_5\in R(4\nu_4)$.

    \item [$R(\bar{\kappa})$] The element $\bar{\kappa}4$ is detected by $g$ in the ASS, and $g_2\in R_{alg}(g)$ with no indeterminacy. Since $g_2$ survives in the $E_{\infty}$-page and detects $\bar{\kappa}_2$, and $h_{\#}(g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-25}$, by Theorem 6.4(c) we deduce that $\bar{\kappa}_2\in R(\bar{\kappa})$.

     \item [$R(2\bar{\kappa})$] The element $2\bar{\kappa}4$ is detected by $h_0g$ in the ASS, and by Corollary 6.12 $h_1g_2\in R_{alg}(h_0g)$ with no indeterminacy. Since $h_1g_2$ survives in the $E_{\infty}$-page and detects $\eta\bar{\kappa}_2$, and $h_{\#}(h_1g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-26}$, by Theorem 6.4(c) we deduce that $\eta\bar{\kappa}_2\in R(\bar{2\kappa})$.

     \item[$R(\eta\bar{\kappa})$] The element $\eta\bar{\kappa}$ is detected by $h_1g$ in the ASS, and by Corollary 6.12 $h_2g_2\in R_{alg}(h_1g)$ with no indeterminacy. Since $h_2g_2$ survives in the $E_{\infty}$-page and detects $\nu\bar{\kappa}_2$, and $h_{\#}(h_2g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-27}$, by Theorem 6.4(c) we deduce that $\nu\bar{\kappa}_2\in R(\eta\bar{\kappa})$.

      \item[$R(\nu\nu_4)$] The element $\nu\nu_4=\sigma^3$ is detected by $h_2^2h_4$ in the ASS, and by Corollary 6.12 $h_3^2h_5=h_4^3\in R_{alg}(h_2^2h_4)$ with no indeterminacy. Since $h_3^2h_5$ survives in the $E_{\infty}$-page and detects $\theta_{4,5}$, and $h_{\#}(h_3^2h_5)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-25}$, by Theorem 6.4(c) we deduce that $\theta_{4,5}\in R(\nu\nu_4)$.

     \item[$R(\eta^2\bar{\kappa})$] The element $\eta^2\kappa$ is detected by $Pd_0$ in the ASS because there is a  hidden $\eta$-extension from $\eta\bar{\kappa}$ to $\{Pd_0\}$, and $gd_1\in R_{alg}(Pd_0)$ with no indeterminacy. Since $gd_1$ survives in the $E_{\infty}$-page and detects $\bar{\kappa}\kappa_1$, and $h_{\#}(gd_1)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-31}$, by Theorem 6.4(c) we deduce that $\bar{\kappa}\kappa_1\in R(\eta^2\bar{\kappa})$.

     \item[$R(\sigma\eta_4)$] The element $\sigma\eta_4$ is detected by $h_4c_0$ in the ASS because there is a  hidden $\sigma$-extension from $h_1h_4$ to $h_4c_0$, and by Corollary 6.12 $h_5c_1\in R_{alg}(h_4c_0)$ with no indeterminacy. Since $h_5c_1$ survives in the $E_{\infty}$-page and $h_{\#}(h_5c_1 )$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-28}$, by Theorem 6.4(c) we deduce that $\{h_5c_1\}\in R(\sigma\eta_4)$.

     \item[$R(\nu\bar{\kappa})$] The element $\nu\bar{\kappa}$ is detected by $h_2g$ in the ASS, and by Corollary 6.12 $h_3g_2\in R_{alg}(h_2g)$ with no indeterminacy. Since $h_3g_2$ survives in the $E_{\infty}$-page and detects $\sigma\bar{\kappa}_2$, and $h_{\#}(h_3g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-29}$ , by Theorem 6.4(c) we deduce that $\sigma\bar{\kappa}_2\in R(\nu\bar{\kappa})$.

     \item[$R(2\nu\bar{\kappa})$] The element $2\nu\bar{\kappa}$ is detected by $h_0h_2g$ in the ASS, and by Corollary 6.12 $h_1h_3g_2\in R_{alg}(h_0h_2g)$ with no indeterminacy. Since $h_1h_3g_2$ survives in the $E_{\infty}$-page and detects $\eta\sigma\bar{\kappa}_2$, and $h_{\#}(h_1h_3g_2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-30}$ , by Theorem 6.4(c) we deduce that $\eta\sigma\bar{\kappa}_2\in R(2\nu\bar{\kappa})$.

     \item[$R(2\rho_{23})$] The element $2\rho_{23}$ is detected by $h_0^3i$ in the ASS, and $\triangle^2h_1h_4\in R_{alg}(h_0^3i)$ with indeterminacy $h_0^2h_3Q_2$. Because $\triangle^2h_1h_4$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-42}$, by Theorem 6.4(c) we deduce that $\{\triangle^2h_1h_4\}\in R(2\rho_{23})$.
     
       \item[$R(4\rho_{23})$] The element $4\rho_{23}$ is detected by $h_0^4i$ in the ASS, and $h_1\triangle^2h_1h_4\in R_{alg}(h_0^4i)$ with indeterminacy $h_0Mg$. Because $h_1\triangle^2h_1h_4$ survives in the $E_{\infty}$-page and $h_{\#}(h_1\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-43}$, by Theorem 6.4(c) we deduce that $\eta\{\triangle^2h_1h_4\}\in R(4\rho_{23})$.
     
      \item[$R(8\rho_{23})$] The element $8\rho_{23}$ is detected by $h_0^5i$ in the ASS, and $h_1^2\triangle^2h_1h_4\in R_{alg}(h_0^5i)$ with no indeterminacy. Because $h_1^2\triangle^2h_1h_4$ survives in the $E_{\infty}$-page and $h_{\#}(h_1^2\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-44}$, by Theorem 6.4(c) we deduce that $\eta^2\{\triangle^2h_1h_4\}\in R(8\rho_{23})$.

      \item[$R(\eta\sigma\eta_4)$] The element $\eta\sigma\eta_4$ is detected by $h_1h_4c_0$ in the ASS and by Corollary 6.12 $h_2h_5c_1\in R_{alg}(h_1h_4c_0)$ with no indeterminacy. Since $h_2h_5c_1$ survives in the $E_{\infty}$-page and $h_{\#}(h_2h_5c_1 )$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-30}$, by Theorem 6.4(c) we deduce that $\nu\{h_5c_1\}\in R(\eta\sigma\eta_4)$.

      \item[$R(\eta\rho_{23})$] The element $\eta\rho_{23}$ is detected by $P^2c_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^2i$ to $P^2c_0$, and $\triangle^2c_1\in R_{alg}(P^2c_0)$ with no indeterminacy. Because $\triangle^2c_1$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-44}$, by Theorem 6.4(c) we deduce that $\{\triangle^2c_1\}\in R(\eta\rho_{23})$.
      
      \item[$R(\eta^2\rho_{23})$] The element $\eta^2\rho_{23}$ is detected by $h_1P^2c_0$ in the ASS because there is a hidden $\eta$-extension from $h_0^2i$ to $P^2c_0$, and $h_2\triangle^2c_1\in R_{alg}(h_1P^2c_0)$ with no indeterminacy. Because $h_2\triangle^2c_1$ survives in the $E_{\infty}$-page and $h_{\#}(h_2\triangle^2h_1h_4)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-46}$, by Theorem 6.4(c) we deduce that $\nu\{\triangle^2c_1\}\in R(\eta^2\rho_{23})$.
      
      \item[$R(\mu_{25})$] The element $\mu_{25}$ is detected by $P^3h_1$ in the ASS, and $\triangle^2h_2g\in R_{alg}(P^3h_1)$ with indeterminacy $Mj$. Because $\triangle^2h_2g$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle^2h_2g)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-67}$, by Theorem 6.4(c) we deduce that $\{\triangle^2h_2g\}\in R(\mu_{25})$.

       \item[$R(\eta\mu_{25})$] The element $\eta\mu_{25}$ is detected by $h_1P^3h_1$ in the ASS, and by Corollary 6.12 $h_2\triangle^2h_2g\in R_{alg}(h_1P^3h_1)$. Because $h_2\triangle^2h_2g$ survives in the $E_{\infty}$-page and $h_{\#}(h_2\triangle^2h_2g)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-69}$, by Theorem 6.4(c) we deduce that $\nu\{\triangle^2h_2g\}\in R(\eta\mu_{25})$.

        \item[$R(\nu^2\bar{\kappa})$] The element $\nu^2\bar{\kappa}$ is detected by $h_2^2g$ in the ASS, and $\triangle_1h_3^2\in R_{alg}(h_2^2g)$ with no indeterminacy. Since $\triangle_1h_3^2$ survives in the $E_{\infty}$-page and $h_{\#}(\triangle_1h_3^2)$ is nontrivial in the $E_{\infty}$-page of the ASS of $P_{-41}$ , by Theorem 6.4(c) we deduce that $\{\triangle_1h_3^2\}\in R(\nu^2\bar{\kappa})$.




        
\end{basedescript}


The $E_r$-page of AHSS is 
\[
E_r^{s,t}=\frac{Im(\pi_t(X^s/X^{s-r})\rightarrow \pi_t(X^s/X^{s-1}))}{Im(\pi_{t+1}(X^{s+r-1}/X^s)\rightarrow \pi_t(X^s/X^{s-1}))}
\]
where the top map is induced by the quotient map
\[
X^s/X^{s-r}\twoheadrightarrow X^s/X^{s-1}
\]
and the bottom map is induced by the attaching map in the cofibre sequence\[
\begin{tikzcd}
X^s/X^{s-1} \arrow[r, hook] & X^{s+r-1}/X^{s-1} \arrow[r, two heads] & X^{s+r-1}/X^s \arrow[r] & \Sigma X^s/X^{s-1}
\end{tikzcd}
\]

Suppose we have a nontrivial differential in the AHSS of $X$: 
\[
d_{s_1-s_2}(\alpha[s_1])=\beta[s_2]\]
where $\alpha\in\pi_*(X^{s_1}/X^{s_1-1})$ and $\beta\in\pi_*(X^{s_2}/X^{s_2-1})$, then we can deduce that the element $\beta[s_2]$ is a permanent cycle in the AHSS of $X^{s_1-1}$. More precisely. if $\beta[s_2]$ supports a nontrivial differential $d_{s_2-s_3}(\beta[s_2]=\gamma[s_3])$ in the AHSS of $X^{s_1-1}$, by the naturality of AHSS we know $\gamma[s_3]$ is trivial in the $E_m$-page of $X$ to avoid the contradiction to the nontrivial differential $d_{s_1-s_2}(\alpha[s_1])=\beta[s_2]$. However, $\gamma[s_3]$ can't support a nontrivial differential or be a target because of the dimension reason. 


\begin{proof}
 Suspend $f$ to the map $\Sigma f:S^{2n}\rightarrow S^{n+1}$, and form its mapping cone $C\Sigma f$. Because suspensions preserve pushouts, there is a homomorphism $C\Sigma f$. We know that $Sq^n:H^n(Cf,\F_2)\rightarrow H^{2n}(Cf,\F_2)$ is nontrivial since $H(f)=1$, and the Steenrod squares are stable cohomology operations, so \[
 Sq^n:H^{n+1}(\Sigma Cf;\F_2)\rightarrow H^{2n+1}(\Sigma Cf;\F_2)
 \]
  is also nontrivial.

 If $\Sigma f$ were homotopic to the constant map, then\[
 \Sigma Cf\simeq C\Sigma f=S^{n+1}\cup_{\Sigma f}D^{2n+1}\simeq S^{n+1}\vee S^{2n+1},
 \]
 so there exists a retraction $r:\Sigma Cf\rightarrow S^{n+1}$. This retraction induces surjections $r^*:H^*(S^{n+1},\F_2)\rightarrow H^*(\Sigma Cf,\F_2)$ on cohomology. By naturality of the Steenrod squares, the following diagram commutes:\[
 \begin{tikzcd}
{H^n(S^{n+1},\F_2)} \arrow[r, "r^*"] \arrow[d, "Sq^n"] & {H^n(\Sigma Cf,\F_2)} \arrow[d, "Sq^n"] \\
{H^{2n}(S^{n+1},\F_2)} \arrow[r, "r^*"]                & {H^{2n}(\Sigma Cf,\F_2)}               
\end{tikzcd}.
 \]
 However, $H^{2n}(S^{n+1},\F_2)=0$, so it implies that $Sq^n\circ r^*=0$, which contradicts to the fact that $r^*$ is surjective and $Sq^n$ is nontrivial on $H^{n+1}(\Sigma Cf,\F_2)$. 

 After taking suspensions repeatedly, we find that $f$ determines a nontrivial class $[f]$ in $\pi^S_{n-1}$.
\end{proof}


\begin{proof}
By the long exact sequence associated with the cofiber sequence:
\[
\begin{tikzcd}
S^{t_2} \arrow[r, hook] & \Sigma^{t_2} C\beta \arrow[r, two heads] & S^{t_1}
\end{tikzcd},
\]
we conclude that \( \alpha[t_1] \) survives in the AHSS of \( \Sigma^{t_2}C\beta \) because \( \alpha \cdot \beta = 0 \). By the naturality of the AHSS induced by the quotient map $T\twoheadrightarrow\Sigma^{t_2}C\beta$, we have the differential in the AHSS of $T$:
\[
d_{t_1-t_2}(\alpha[t_1])=0
\]
Consider any element in $\pi_{t_0+t_1}(\Sigma^{t_2}C\beta)$ detected by $\alpha[t_1]$ since $\alpha[t_1]$ survives. We abuse the notation to denote such an element by $\alpha[t_1]$. By the definition of Toda bracket $\langle\alpha,\beta,\gamma\rangle$, the class $a_{2*}(\alpha[t_1])$ is an element in $\langle\alpha,\beta,\gamma\rangle[t_3]$.

\[\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Ellipse [id:dp5909860694640758] 
\draw   (146,180.65) .. controls (146,178.59) and (148.07,176.92) .. (150.63,176.92) .. controls (153.18,176.92) and (155.26,178.59) .. (155.26,180.65) .. controls (155.26,182.71) and (153.18,184.38) .. (150.63,184.38) .. controls (148.07,184.38) and (146,182.71) .. (146,180.65) -- cycle ;
%Shape: Ellipse [id:dp7243812852572209] 
\draw   (313.41,210.68) .. controls (313.41,208.62) and (315.48,206.95) .. (318.04,206.95) .. controls (320.59,206.95) and (322.67,208.62) .. (322.67,210.68) .. controls (322.67,212.74) and (320.59,214.4) .. (318.04,214.4) .. controls (315.48,214.4) and (313.41,212.74) .. (313.41,210.68) -- cycle ;
%Shape: Ellipse [id:dp8503380837958581] 
\draw   (229.31,210.78) .. controls (229.31,208.67) and (231.44,206.95) .. (234.07,206.95) .. controls (236.7,206.95) and (238.83,208.67) .. (238.83,210.78) .. controls (238.83,212.9) and (236.7,214.62) .. (234.07,214.62) .. controls (231.44,214.62) and (229.31,212.9) .. (229.31,210.78) -- cycle ;
%Shape: Ellipse [id:dp3953588264660117] 
\draw   (237.52,179.03) .. controls (238.11,181.03) and (236.58,183.04) .. (234.09,183.52) .. controls (231.61,183.99) and (229.11,182.76) .. (228.51,180.76) .. controls (227.92,178.76) and (229.45,176.75) .. (231.94,176.27) .. controls (234.43,175.79) and (236.92,177.02) .. (237.52,179.03) -- cycle ;
%Straight Lines [id:da7978209120620792] 
\draw    (234.09,183.52) -- (234.07,206.95) ;
%Straight Lines [id:da5940100576732934] 
\draw    (155.26,180.65) -- (226.51,180.76) ;
\draw [shift={(228.51,180.76)}, rotate = 180.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9931591544149998] 
\draw    (238.83,210.78) -- (311.41,210.68) ;
\draw [shift={(313.41,210.68)}, rotate = 179.92] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (188.4,169.51) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (235.31,185.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \beta $};
% Text Node
\draw (272.42,198.26) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \gamma $};


\end{tikzpicture}
\]
The indeterminacy of the Toda bracket is $\alpha\cdot\pi_{t_1-t_3-1}+\gamma\cdot\pi_{t_0+t_1-t_2}$. From the construction of the AHSS, $a_{2*}(\alpha[t_1])$ is also a representative for $d_{t_1-t_3}(\alpha[t_1])$.
\[
\begin{tikzcd}
S^{t_0+t_1} \arrow[r] & \Sigma^{t_2}C\beta \arrow[r, "a_2"] & \Sigma S^{t_3}
\end{tikzcd}
\]
The indeterminacy of the target of this differential is the image of
\[d_{t_2-t_3}: \pi_{t_0+t_1-t_2+t_3+1}(S^{t_2})\rightarrow\pi_{t_0+t_1}(\Sigma S^{t_3}),\]
which is $\gamma\cdot\pi_{t_0+t_1-t_2+t_3+1}$, since it's induced by the multiplication of $\gamma$ map. So we have $d_{t_1-t_3}(\alpha[t_1])\subseteq\langle\alpha,\beta,\gamma\rangle[t_3]$.

If $\alpha\cdot\pi_{t_1-t_3-1}\subseteq\gamma\cdot\pi_{t_0+t_1-t_2}$, then $d_{t_1-t_3}(\alpha[t_1])$ and $\langle\alpha,\beta,\gamma\rangle[t_3]$ have a
 common element and have the same indeterminacy, so we have $d_{t_1-t_3}(\alpha[t_1])=\langle\alpha,\beta,\gamma\rangle[t_3]$.
 

\end{proof}




\begin{lemma}\cite[Lemma 6.1]{wang2017triviality61stemstablehomotopy}
Let \( T \) be a three-cell complex with cells in dimensions \( t_1, t_2, t_3 \), where \( t_3 < t_2 < t_1 \). Suppose we have cofiber sequences:
\[
\begin{tikzcd}
\Sigma^{t_3}C\gamma \arrow[r, "i_1", hook] & T \arrow[r, "q_1", two heads] & S^{t_1} \arrow[r, "a_1"] & \Sigma^{t_3+1}C\gamma
\end{tikzcd}
\]

\[
\begin{tikzcd}
S^{t_3} \arrow[r, "i_2", hook] & T \arrow[r, "q_2", two heads] & \Sigma^{t_2}C\beta \arrow[r, "a_2"] & \Sigma S^{t_3}
\end{tikzcd},
\]
where $C\gamma$ is the cofibre of $\gamma\in\pi_{t_2-t_3-1}$ , $C\beta$ is the cofibre of $\beta\in\pi_{t_1-t_2-1}$ and $\gamma, \beta$ are nontrivial classes such that $\gamma\cdot\beta=0$. In other words, the cell diagram of $T$ is the following:

\[\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Ellipse [id:dp7147761916872644] 
\draw   (335.91,256.2) .. controls (335.91,250.2) and (341.08,245.33) .. (347.46,245.33) .. controls (353.83,245.33) and (359,250.2) .. (359,256.2) .. controls (359,262.21) and (353.83,267.08) .. (347.46,267.08) .. controls (341.08,267.08) and (335.91,262.21) .. (335.91,256.2) -- cycle ;
%Straight Lines [id:da9349613491753661] 
\draw    (347.46,267.08) -- (346.68,311.5) ;
%Shape: Ellipse [id:dp4092725737428382] 
\draw   (335.21,322.3) .. controls (335.21,316.33) and (340.34,311.5) .. (346.68,311.5) .. controls (353.01,311.5) and (358.15,316.33) .. (358.15,322.3) .. controls (358.15,328.27) and (353.01,333.1) .. (346.68,333.1) .. controls (340.34,333.1) and (335.21,328.27) .. (335.21,322.3) -- cycle ;
%Straight Lines [id:da6541312554049883] 
\draw    (346.68,333.1) -- (346.68,378.32) ;
%Shape: Ellipse [id:dp2407729602560431] 
\draw   (336.06,388.33) .. controls (336.06,382.8) and (340.81,378.32) .. (346.68,378.32) .. controls (352.54,378.32) and (357.3,382.8) .. (357.3,388.33) .. controls (357.3,393.85) and (352.54,398.33) .. (346.68,398.33) .. controls (340.81,398.33) and (336.06,393.85) .. (336.06,388.33) -- cycle ;

% Text Node
\draw (342.84,247.14) node [anchor=north west][inner sep=0.75pt]   [align=left] {$ $};
% Text Node
\draw (331.48,280.05) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \beta $};
% Text Node
\draw (341.1,315.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle t_{2}$};
% Text Node
\draw (341.95,247.64) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle t_{1}$};
% Text Node
\draw (340.1,381.3) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle t_{3}$};
% Text Node
\draw (330.33,343.48) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \gamma $};


\end{tikzpicture}
\]

Suppose the class $\alpha\in\pi_{t_0}$ satisfies the condition $\alpha\beta=0$ in $\pi_{t_0+t_1-t_2-1}$. Then we have an Atiyah-Hirzebruch differential:
\[
d_{t_1-t_3}(\alpha[t_1])\subseteq\langle\alpha,\beta,\gamma\rangle[t_3]
\]
If moreover $\alpha\cdot\pi_{t_1-t_3-1}\subseteq\gamma\cdot\pi_{t_0+t_1-t_2}$, then we have an Atiyah-Hirzebruch differential:
\[
d_{t_1-t_3}(\alpha[t_1])=\langle\alpha,\beta,\gamma\rangle[t_3].
\]

\end{lemma}





\appendix

In the appendix we recall the theory of cell diagram which is useful when thinking of finite CW spectra described in \cite{10.1007/BFb0078740}. We will also recall the definition of Toda bracket and Massey product and present the Moss convergence theorem.
\section{Cell Diagrams, Toda Brackets, and the Moss Convergence Theorem}
\begin{definition}
Let \( Z \) be a finite CW spectrum. A cell diagram for \( Z \) consists of nodes and edges. The nodes are in one-to-one correspondence with a chosen basis of the mod \( 2 \) homology of \( Z \), and they may be labeled with symbols to indicate their dimensions. When two nodes are joined by an edge, it is possible to form an \( HF_2 \)-subquotient \( Z'/Z'' = S^n \cup_f e^m \).
\end{definition}
\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Shape: Circle [id:dp1029919650851332] 
\draw   (329,189.5) .. controls (329,183.7) and (333.7,179) .. (339.5,179) .. controls (345.3,179) and (350,183.7) .. (350,189.5) .. controls (350,195.3) and (345.3,200) .. (339.5,200) .. controls (333.7,200) and (329,195.3) .. (329,189.5) -- cycle ;
%Shape: Circle [id:dp13558643285387806] 
\draw   (329,250.5) .. controls (329,244.7) and (333.7,240) .. (339.5,240) .. controls (345.3,240) and (350,244.7) .. (350,250.5) .. controls (350,256.3) and (345.3,261) .. (339.5,261) .. controls (333.7,261) and (329,256.3) .. (329,250.5) -- cycle ;
%Straight Lines [id:da9150702236703705] 
\draw    (339.5,200) -- (339.5,240) ;

% Text Node
\draw (332,184) node [anchor=north west][inner sep=0.75pt]   [align=left] {m};
% Text Node
\draw (335,245) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {n};
% Text Node
\draw (330,213) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle f$};


\end{tikzpicture}
\]
The cells in the subcomplex \( Z' \) but not in \( Z'' \) correspond precisely to the two nodes, and the attaching map is the map \( f \) shown.

\begin{definition}
Given \( \alpha, \beta, \gamma \in \pi^s_* \) such that \( \alpha \cdot \beta = 0 \) and \( \beta \cdot \gamma = 0 \), the Toda bracket of \( \alpha, \beta, \gamma \) is the set \( \langle \alpha, \beta, \gamma \rangle \) defined as follows:

Since \( \alpha \cdot \beta = 0 \) and \( \beta \cdot \gamma = 0 \), we have the following diagram:
\[
\begin{tikzcd}
& \Sigma^{|\gamma|-1}C\beta \arrow[d] & \\
S^{|\alpha|+|\beta|+|\gamma|} \arrow[r, "\alpha"] \arrow[ru, "f", dashed] & S^{|\beta|+|\gamma|} \arrow[r, "\beta"] & S^{|\gamma|} \arrow[r, "\gamma"] \arrow[d] & S^0 \\
& & \Sigma^{|\gamma|}C\beta \arrow[ru, "g"', dashed] & 
\end{tikzcd}
\]
The Toda bracket \( \langle \alpha, \beta, \gamma \rangle \) is then defined as:
\[
\langle \alpha, \beta, \gamma \rangle := \{ g \circ \Sigma f : S^{|\alpha|+|\beta|+|\gamma|+1} \rightarrow S^0 \mid f \text{ and } g \text{ are elements of } \pi_*^s \text{ such that the diagram commutes} \}.
\]
\end{definition}

The indeterminacy of \( \langle \alpha, \beta, \gamma \rangle \) is defined as the set of differences between any two elements in \( \langle \alpha, \beta, \gamma \rangle \). By definition, the indeterminacy is given by:
\[
\pi_{|\alpha|+|\beta|+1} \cdot \gamma + \alpha \cdot \pi_{|\beta|+|\gamma|+1}.
\]

Let $R$ be a differential graded $\Z_2$-algebra with $d:R^n\rightarrow R^{n+1}$, and the cohomology of $R$ is $H^*(R)$.
\begin{definition}
Let \( [x_0], [x_1], [x_2] \in H^*(R) \) be such that \( [x_0][x_1] = 0 \) and \( [x_1][x_2] = 0 \). Then there exist \( x_{01}, x_{12} \in R \) satisfying \( dx_{01} = x_0 x_1 \) and \( dx_{12} = x_1 x_2 \). Since \( d(x_{01}x_2 + x_0 x_{12}) = 2x_0 x_1 x_2 = 0 \), the element \( x_{01}x_2 + x_0 x_{12} \) is a cycle. The Massey product of \( [x_0], [x_1], [x_2] \) is defined as the set:
\[
\langle [x_0], [x_1], [x_2] \rangle := \{ [x_{01}x_2 + x_0 x_{12}] \mid x_0, x_1, x_2 \text{ represent } [x_0], [x_1], [x_2] \text{ and } dx_{01} = x_0 x_1, dx_{12} = x_1 x_2 \}.
\]
\end{definition}

It's easily verified that $[x_{01}x_2+x_0x_{12}]$ is independent of the choice of $x_0,x_1,x_2$, so $\langle[x_0],[x_1],[x_2]\rangle$ is well defined if the set is nonempty.

Moss convergence theorem tells us the relationship between Toda brackets and Moss products.
\begin{theorem}\cite[Moss Convergence Theorem]{Moss}
Let \( \{E_r, d_r\} \) be a spectral sequence converging to the stable homotopy groups \( \pi_* \). Suppose \( a, b, c \in E_r \) satisfy the following conditions:
\begin{enumerate}
    \item \( a, b, c \) are permanent cycles.
    \item They detect \( \alpha, \beta, \gamma \in \pi_* \), respectively.
    \item The Massey product \( \langle a, b, c \rangle \) is defined on the \( E_r \)-page.
    \item The Toda bracket \( \langle \alpha, \beta, \gamma \rangle \) is defined in \( \pi_* \).
    \item There are no crossing differentials for the products \( ab = 0 \) and \( bc = 0 \).
\end{enumerate}
Then there exists an element in \( \langle a, b, c \rangle \) on the \( E_r \)-page that is a permanent cycle and detects an element in \( \langle \alpha, \beta, \gamma \rangle \).
\end{theorem}
 Here ``no crossing differential" means the following case won't happen in the $E_r$-page:\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,502); %set diagram left start at 0, and has height of 502

%Straight Lines [id:da8597464575944997] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (168,263.22) -- (139.06,168.39) ;
\draw [shift={(138.48,166.48)}, rotate = 73.03] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6559552069069874] 
\draw    (167,231.22) -- (136.98,192.08) ;
\draw [shift={(135.76,190.49)}, rotate = 52.51] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (126.99,176.23) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \cdot $};
% Text Node
\draw (126.99,152.23) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \cdot $};
% Text Node
\draw (166.89,265) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \cdot $};
% Text Node
\draw (166.89,227.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \cdot $};
% Text Node
\draw (114.07,182.92) node [anchor=north west][inner sep=0.75pt]   [align=left] {ab};
% Text Node
\draw (156.31,202.52) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle d_{r}{}_{- 1}$};


\end{tikzpicture}
 \]



Here is an equivalent definition of Mahowald invariant.
\begin{proposition}
[An alternative definition of Mahowald invariant, \cite{Hill2004EquivariantMahowald}]
Let \( C_2 \) denote the cyclic group of order 2. Fix a specific representation \( \xi \) as the sign representation (and its one-point compactification) of \( S \). Consider the diagram:
\[
\begin{tikzcd}
                                         &                                                                & S^{n+({k+1})\xi} \\
                                         & S^{n+k\xi} \arrow[rd, "M_\xi(\alpha)", dashed] \arrow[ru, "j"] &                  \\
S^n \arrow[rr, "\alpha"] \arrow[ru, "i"] &                                                                & S^0             
\end{tikzcd}
\]
so that $M_\xi(\alpha)$ exists, but it can't be lifted through $j$ . Define the $C_2$- equivariant Mahowald invariant $M_{c_2}(\alpha)=M_\xi(\alpha)$ to be the dashed line ($G$-equivariant) that fill the diagram. We have $M(\alpha)=M_{c_2}(\alpha)$.
\end{proposition}
In fact, when the group $G$ is not $C_2$, we can also define the $G$-equivariant Mahowald invariant. So it generalizes the original definition of Mahowald invariant.
By this theorem, we have a simple way to prove the following theorem:


\begin{theorem}\cite{Quigley_2021}\label{4.7}
For $\alpha\in\pi_*$, $|M(\alpha)|\geq2|\alpha|$ 
\end{theorem}
\begin{proof}
The notations are as above. There is a diagram:
\[
\begin{tikzcd}
                                                   & S^n\wedge{S^{n\xi}}=S^{n+n\xi} \arrow[rd, "\alpha\wedge\alpha", dashed] &     \\
S^n \arrow[rr, "\alpha"] \arrow[ru, "id\wedge{0}"] &                                                                         & S^0.
\end{tikzcd}
\]
So degree of i is equal or bigger than n,
So $|M(\alpha)|$ is at least $2|\alpha|$.
\end{proof}



If $\alpha$ is represented by a map
$f:S^{n-1}\rightarrow S^{-1}$, the composition with the inclusion $i:S^{-1}\rightarrow P^{\infty}_{-1}$ is null homotopic, provided that $f$ is not a unit multiple of identity map. It is because we have the cofibration:\[
\begin{tikzcd}
\Sigma^{-1}P_0^{\infty} \arrow[r] & S^{-1} \arrow[r] & P_{-1}^{\infty}
\end{tikzcd}.
\]
 The lefthand map is studied by Kahn-Priddy \cite{Kahn_Priddy_1978} and they show that the cokernel of the induced map in homotopy groups is $\Z_2$ generated by fundamental class. So we know $N>1$, and $M(\alpha)$ is a subset of $\pi_{n+N-1}(S^0)$.


 \begin{definition}
Let $f:S^{2n-1}\rightarrow S^n$, and let $Cf$ denote its mapping cone. Let $\alpha$ and $\beta$ be generators of $H^n(Cf,\F_2)$ and $H^{2n}(Cf,\F_2)$ respectively. The \textit{mod 2 Hopf invariant of f} is defined to be the integer $H(f)\in \{0,1\}$ such that \[
Sq^n(\alpha)=H(f)\beta.
\]
\end{definition}

Since the Steenrod squares are stable cohomology operations, the following proposition shows that a map with Hopf invariant one yields a nontrivial element in the stable homotopy groups of spheres:
\begin{proposition}\cite[Ch. 4]{adams1974stable}
Suppose $f:S^{2n-1}\rightarrow S^n$ has Hopf invariant one. Then $f$ determines a nontrivial class $[f]\in\pi^S_{n-1}$, the $(n-1)-$stem of the stable homotopy groups of spheres.
\end{proposition}

Therefore, we have a question: for which value of $n$ does there exist a map $f:S^{2n-1}\rightarrow S^n$ with mapping cone $Cf$ such that $Sq^n$ connects the bottom cell and the top cell of $Cf$ in $\F_2$-cohomology?
For such map $f$ and $n$, the extension\[
\begin{tikzcd}
0 \arrow[r] & {H^*(S^{2n},\F_2)} \arrow[r] & {H^*(Cf,\F_2)} \arrow[r] & {H^*(S^n,\F_2)} \arrow[r] & 0
\end{tikzcd}
\]does not split as a short exact sequence of $\mathcal{A}$-modules. So $f$ represents a nontrivial class in $\Ext^{s,t}_{\mathcal{A}}(\F_2,\F_2)$.

From the last subsection, we know that $h_i\in\Ext^{1,2^i}_{\mathcal{A}}(\F_2,\F_2)$ is the generator dual to $Sq^{2^i}\in\mathcal{A}$ for any non-negative integer $i$, so we deduce that $Sq^{2^i}$ detects the corresponding attaching map for $i=0,...,3$ in the cofiber of these maps with Hopf invariant one.


\begin{proof}
We assume that \( u \) is a nontrivial permanent cycle in the \( E_2 \)-page and detects the homotopy map \( f \). However, \( M_{alg}(u) \) may fail to contain a permanent cycle. Consider the following diagram of \( \Ext \) groups:
\begin{equation}\label{2}
\begin{tikzcd}
E_2(S^{t-1}) \arrow[r, "v"] \arrow[d, "u"'] & E_2(S^{-n}) \arrow[d, "i_*"'] & \\
E_2(S^{-1}) \arrow[r, "h_{\#}"] & E_2(P^{\infty}_{-n}) \arrow[r, "j_{\#}"] & E_2(P^{\infty}_{-n+1})
\end{tikzcd}.
\end{equation}
Suppose $n$ is not the smallest with respect to the property that $h\circ f$ is nontrivial, which can happen when $j\circ h\circ f$ is essential but has higher Adams filtration than expected. In this case, we can't get the following commutative diagram:
\begin{equation}\label{1}
\begin{tikzcd}
S^{-1+t} \arrow[r, "g"] \arrow[d, "f"'] & S^{-n} \arrow[d, "i"']         &                   \\
S^{-1} \arrow[r, "h"]                   & P^{\infty}_{-n} \arrow[r, "j"] & P^{\infty}_{-n+1}
\end{tikzcd}
\end{equation}
and $M_{alg}(u)$ does not contain a permanent cycle, and the homotopy Mahowald invariant $M(f)$ has smaller stems than the algebraic Mahowald invariant $M_{alg}(u)$.

On the other hand, if $n$ is the smallest with respect to the property that $h\circ f$ is nontrivial, then the commutative diagram \ref{1} exists, and $M(f)$ and $M_{alg}(u)$ are in the same stem. However, $h_{\#}(u)$ may be the target of a nontrivial differential, so the map $i\circ g=h\circ f $ has higher Adams filtration and the coset $M(f)$ has higher Adams filtration than the algebraic Mahowald invariant $M_{alg}(u)$.

If $h_{\#}(u)$ can survive in the $E_{\infty}$-page and $j\circ h\circ f$ is null, then $M_{alg}(u)$ contains a permanent cycle represented by $g$. Since each choice of $g$ in \ref{1} is represented by some $v$ in \ref{2}, we have the relation:
\[
M(f)\subset\{M_{alg}(u)\}.
\]

Finally, if $h\circ f$ is null (this could happen if $h_{\#}(u)$ is the target of a nontrivial differential), then $M(f)$ is in a larger stem than $M_{alg}(u)$.
\end{proof}


The construction of the algebraic Atiyah-Hirzebruch spectral sequence (AAHSS) is similar to that of the AHSS. Let $X$ be a spectrum. There is a filtration on $H^*(X)$ by the degrees. For any $n$ there is a short exact sequence\[
\begin{tikzcd}
0 \arrow[r] & H^{\geq n+1}(X) \arrow[r] & H^{\geq n}(X) \arrow[r] & H^n(X) \arrow[r] & 0
\end{tikzcd}.
\]
This induces a long exact sequence:\[
\begin{tikzcd}
\cdots \arrow[r] & \Ext(\F_2)\otimes H^n(X) \arrow[r] & \Ext(H^{\geq n}(X)) \arrow[r] & \Ext(H^{\geq n+1}(X)) \arrow[r] & \cdots.
\end{tikzcd}
\]
 Combining the long exact sequences for all $n$, we get the algebraic Atiyah-Hirzebruch spectral sequence:
\[
\oplus_n\Ext(\F_2)\otimes H^*(X)\Rightarrow \Ext(H^*(X)).
\]

\begin{proposition}\label{5.13}
$\{\triangle h_1h_3\}\in M(\eta_4)$ 
\end{proposition}
\begin{proof}
 The element $\eta_4$ is detected by $h_1h_4$ in the ASS. By Corollary \ref{3.11}, $h_2h_5\in M_{alg}(h_1h_4)$ with no indeterminacy, and we know $h_2h_5\in R^{[2]}_{HF_2}(\eta_4)$ by Theorem \ref{3.9}. We have the Adams differential $d_3(h_2h_5)=h_0p$, and we have $\langle P^{-18}_{-19}\rangle p=h_0p$ by Theorem \ref{3.8}, so we know $p\in R^{[4]}_{HF_2}(\eta_4)$. By $|\eta_4|=16$ and Theorem \ref{3.4}(a), we deduce that $32\leq|M(\eta_4)|\leq33$. By Theorem \ref{3.6}, it suffices to check the generators of $\pi_{32}$ and $\pi_{33}$ with filtrations greater than $4$. 
 
 In the AHSS of $P_{-17}$, we have \[
 d_2(\{h_0^{10}h_5\}[-15])=\{P^3c_0\}[-17],\]
 because there is a hidden $\eta$-extension. In the AHSS of $P_{-18}$, we have
 \[d_4(\theta_4[-14])=\{p\}[-18],\]
 because there is a hidden $\nu$-extension. And we have
 \[d_2(\{\triangle h_1h_3\}[-16])=\eta\{\triangle h_1h_3\}[-18], d_2(\{P^3c_0\}[-16])=\eta\{P^3c_0\}[-18].\] 
 So we know that the only nontrivial element in homotopy groups is $\{\triangle h_1h_3\}[-17]$ and we deduce that $\{\triangle h_1h_3\}\in M(\eta_4)$. 
\end{proof}

\begin{proposition}\label{5.17}
 $\nu\bar{\kappa}_2\in M(\nu\bar{\sigma})$   
\end{proposition}
\begin{proof}
The element $\nu\bar{\sigma}$ is detected by $h_2c_1$ in the ASS, and $h_3c_2\in M_{alg}(h_2c_1)$. By Theorem \ref{3.9} we know $h_3c_2\in R^{[4]}_{HF_2}(\nu\bar{\sigma})$. We have the Adams differential $d_2(h_3c_2)=h_0h_2g_2$, and by Theorem \ref{3.8} we have $\langle P^{-26}_{-27}\rangle h_3g_2=h_0h_3g_2$, so by Theorem \ref{3.8} we know $h_2g_2\in R^{[5]}_{HF_2}(\nu\bar{\sigma})$. By $|\nu\bar{\sigma}|=2$ and Theorem \ref{3.4}(a), we deduce $44\leq|M(\nu\bar{\sigma})|\leq 47$. By Theorem \ref{3.6} it suffices to check the generators of $\pi_{44}$,$\pi_{45}$ and $\pi_{46}$ with filtrations greater than 5.

Since $|M(\bar{\sigma})|\geq 38$, by Theorem \ref{3.12} we have \[M(\nu\bar{\sigma})\geq 38+|M(\nu)|=45.\]
In the AHSS of $P^\infty_{-25}$, we have Atiyah-Hirzebruch differentials \[\begin{split}
   & d(\{h_5d_0\}[-23])=\eta\{h_5d_0\}[-25],d(\eta\bar{\kappa}_2[-23])=\eta^2\bar{\kappa}_2[-25],\\
   & d(\theta_{4,5}[-23])=\{Mh_1\}[-25]\; \mathrm{and}\; d(\{\triangle h_1g\}[-23])=\{d_0l\}[-25].
\end{split} \] 
They are all candidates of 46-stem, so $|M(\nu\bar{\sigma})|\neq 46$. 

If $|M(\nu\bar{\sigma})|=45$, we have \[M(\bar{\sigma})+M(\nu)\geq 38+7=45,\] so we have 
$M(\nu)M(\bar{\sigma})\subseteq M(\nu\bar{\sigma})$. Similarly, we know $c_2\in M_{alg}(c_1)$, so $f_1\in R^{[4]}_{HF_2}(\bar{\sigma})$. By Theorem \ref{3.6}, the only possibility of $M(\bar{\sigma}) $ with a $\sigma$-extension is $\{h_0^3h_3h_5\}$. However, in the AHSS of $P_{-24}$ we have an Atiyah-Hirzebruch differential 
\[d(\{h_0^3h_3h_5\}[-16])=8\theta_{4,5}[-24],\] so $\sigma\{h_0^3h_3h_5\}\notin M(\nu\bar{\sigma})$, which is a contradiction.

Therefore, all candidates of 44-stem to 46-stem are impossible and we deduce $\nu\bar{\kappa}_2\in M(\nu\bar{\sigma})$.
\end{proof}
